MOSAIC: Efficient Mixture-of-Agent Scheduling via Adaptive Aggregation and Inference Concurrency

Mixture-of-Agents (MoA) systems improve reasoning accuracy by routing each query to multiple expert LLMs and aggregating their outputs. Efficiently executing this workload on limited GPU resources has bottlenecks. Skill-based routing creates skewed expert demand, and combining instruction-tuned LLMs with long-reasoning models results in extreme variability in generation lengths. Consequently, traditional scheduling strategies suffer from significant GPU idling and throughput collapse due to load imbalances. We present MOSAIC, a scheduling framework for accelerating batch-oriented MoA workloads. MOSAIC uses two-stage workload-aware scheduling: an expert placement stage, where an integer linear program (ILP) decides expert placement, followed by a query-sequencing stage that schedules requests based on predicted output lengths. Additionally, MOSAIC uses confidence-aware adaptive aggregation, leveraging inter-expert agreement to bypass the heavy aggregator LLM for consensus queries. On a 4-GPU system, MOSAIC achieves 2.7-3.4x end-to-end speedups over round-robin scheduling and reduces the mean time-to-answer by 3.9-7.8x, while matching accuracy within +/-1pp.

==> Sections/02_Background.tex <==
\section{Background and and Related Works}
\label{sec:background}

% \textbf{Or do Background and Related works here and a motivation section next???}
%\SK{Clearly define your 'Mixture of Agent' first, and then talk about the literature... so that the reader does not confuse with agentic multimodel, as we still are doing inference only monolithic inference...that is different from current standard definition of agents, and does not involve any tool call in our assumption.}
Multi-model multi-agent, relevance in complex reasoning task
Self consistency
MoA
self MoA
SLM-MUX
Symbolic-MoE

realtime-serving
offline-serving
Alpaserve
Muxserve




==> Sections/03_Motivation.tex <==
\section{Motivational Case Studies}
\label{sec:motivation}

% Fundamental knowledge needed to understand this paper


% Few lines what case studies we are looking at

\insertFigure{tokenskew2} {Overview figure.}

\addnt{Need a smoother transition from the previous section. Revisit after finishing writing the previous section}
% 1. Factors resposible to make RR allocation skewed
In a multi-GPU environment, a naive static scheduler assigns one expert model per GPU worker. It executes all the questions that require that model as a solver, to prevent frequent model offloading. This setup suffers from severe GPU idling due to the following reasons:


% \SM{get the numbers avaible on respective figures}

% % a. output token skew
% \betterparagraph{1. Heterogeneous Token-Budget Profiles Across Solver Classes} 
% % There is large disparity in output-token cost between reasoning and non-reasoning models.
% Reasoning models have a significantly higher output-token cost compared to non-reasoning models.
% %
% For MMLU-pro, when tested across 12 models (6 reasoning, 6 non-reasoning) with diverse recruitment scenarios, reasoning-based models generate a median of 3289 tokens per prompt, almost  6.3$\times$ more than non-reasoning models (518 tok/prompt), as seen in \autoref{fig:tokenskew2}a.
% %
% The variable length of chain-of-thought (CoT) traces is reflected in the wide distribution of token lengths(\textasciitilde1500 to \textasciitilde6000).
% %
% % In the LLM decode phase, token generation is the dominant component in overall inference latency.
% %
% % Tokens are a faithful proxy for compute expenditure, as average generation time per prompt scales linearly with output tokens across solvers (\autoref{fig}).
% %
% % The latency is also model architecture dependent.
% %
% % For example QwenR1, being more verbose, generates more tokens (3734) on average than LLamaR1 (3146).
% %
% % But it is more efficient, resulting in shorter response times per prompt on average.

% Also, a solver's token-budget profile is not static but dependent on the composition of the broader solver pool (\autoref{fig:tokenskew2}b).
% %
% In the default mixed pool, LlamaR1 and QwenR1 are the only reasoning-capable solvers.
% %
% So the skill-based router implicitly performs difficulty routing, allocating reasoning-intensive questions (multi-step derivation, quantitative analysis) to them.
% %
% Naturally in this configuration, LLamaR1 and QwenR1 generates 3146 and 3734 tokens per prompt on average respectively.
% %
% To isolate this effect, we consider a synthetic all reasoning-model pool (allR).
% %
% Here they must compete against four additional R1 distillations for a solver slot.
% %
% Now they get a broader, mixed-difficulty subset of questions where their specific profile excels, with their token costs per prompt dropping to 2302 (-27\%) and 2522 (-32\%).
% %
% Meanwhile, the most-demanding questions migrate to specialized long-CoT solvers (SkyworkR1: 5339 tok/prompt; StratosR1: 5822 tok/prompt).
% %
% This confirms that the compute profile of a model is dynamically shaped by its peers.


% a. output token skew
\betterparagraph{Observation 1}\textit{Heterogeneous model categories and solver pools yield highly diverse generation token count, with LRMs often showing long tail distribution of token count across candidate solvers.}

\noindent
\autoref{fig:tokenskew2}(a) summarizes an experiment with MMLU-Pro, across 12 models of different classes (6 reasoning and 6 non-reasoning).
%
The LRMs' average generation length (3289 tokens/prompt) is $6.3\times$ longer than that of an LLM (518 tokens/prompt).
%
Further, LRMs often show long tail distribution of token generation, ranging from 1500 to 6000 tokens per prompt.
%(in \autoref{fig:tokenskew2}(a) it ranges from 1500 to 6000).
%
Additionally, the token-budget profile of a solver is not static but dependent on the composition of the broader solver pool.
%
\autoref{fig:tokenskew2}b shows two different solver pools, the default has two LRMs and four LLMs while the all reasoning (allR) pool has all six solver candidates as LRMs.
%
In default pool, LLamaR1 and QwenR1 being the only LRMs, generate 3146 and 3734 tokens per prompt on average respectively.
%
But on allR, they get a broader, mixed-difficulty subset of questions where their specific profile excels, with their token costs per prompt dropping to 2302 (-27\%) and 2522 (-32\%).
%
Meanwhile, the most-demanding questions migrate to specialized long-CoT solvers (Skywork: 5339 tokens/prompt; Stratos: 5822 tokens/prompt).
%
\textbf{This confirms that the compute profile of a model is dynamically shaped by its peers}.
\addnt{This confirms that a model’s compute profile is dynamically shaped by its peers, since the solver pool affects the difficulty of the questions routed to that model.}


% There is large disparity in output-token cost between reasoning and non-reasoning models.

%Reasoning models have a significantly higher output-token cost compared to non-reasoning models.
%
%For MMLU-pro, when tested across 12 models (6 reasoning, 6 non-reasoning) with diverse recruitment scenarios, reasoning-based models generate a median of 3289 tokens per prompt, almost  6.3$\times$ more than non-reasoning models (518 tok/prompt), as seen in \autoref{fig:tokenskew2}a.
%
%The variable length of chain-of-thought (CoT) traces is reflected in the wide distribution of token lengths(\textasciitilde1500 to \textasciitilde6000).

%
% In the LLM decode phase, token generation is the dominant component in overall inference latency.
%
% Tokens are a faithful proxy for compute expenditure, as average generation time per prompt scales linearly with output tokens across solvers (\autoref{fig}).
%
% The latency is also model architecture dependent.
%
% For example QwenR1, being more verbose, generates more tokens (3734) on average than LLamaR1 (3146).
%
% But it is more efficient, resulting in shorter response times per prompt on average.

%Additionally, a solver's token-budget profile is not static but dependent on the composition of the broader solver pool (\autoref{fig:tokenskew2}b).
%
%In the default mixed pool, LlamaR1 and QwenR1 are the only reasoning-capable solvers.
%
%So the skill-based router implicitly performs difficulty routing, allocating reasoning-intensive questions (multi-step derivation, quantitative analysis) to them.
%
%Naturally in this configuration, LLamaR1 and QwenR1 generates 3146 and 3734 tokens per prompt on average respectively.
%
%To isolate this effect, we consider a synthetic all reasoning-model pool (allR).
%
%Here they must compete against four additional R1 distillations for a solver slot.
%
%Now they get a broader, mixed-difficulty subset of questions where their specific profile excels, with their token costs per prompt dropping to 2302 (-27\%) and 2522 (-32\%).
%
%Meanwhile, the most-demanding questions migrate to specialized long-CoT solvers (SkyworkR1: 5339 tok/prompt; StratosR1: 5822 tok/prompt).
%
%This confirms that the compute profile of a model is dynamically shaped by its peers.

% b. expert selection skew
% Another important contributor to workload imbalance is the uneven popularity of solvers depending on the skill-level weighted sampling from the model pool. For the default model mix (reasoning and non-reasoning) in MMLU-pro (2100 questions in the test set, in total having 6300 solver selected), the solver that was selected least was Exaone (547 times) and Gemma being the most popular (1632). We plot the coefficient of variance plot across all solvers and max/min value is also provided. When R1s are removed from the pool, the strongest remaining models (Gemma 53%, Qwen 24%) dominate while Llama/Granite get <2% of slots each. max/min ratio = 92× — the popularity skew is much worse than the original 2.98×.


% \insertWideFigure{popularity}{Overview figure.}
\insertWideFigureShrink{popularity2}{Overview figure.\SM{reduce height}}{1}
% \betterparagraph{II. Solver Popularity Skew} 
% \SK{follow earlier style and make it precise and to the point.}

\betterparagraph{Observation 2}
\textit{Popularity of different solvers across model pools largely vary as a result of skill-weighted sampling by the router.}
\noindent
% Another major contributor to workload imbalance is the uneven popularity of solvers under skill-weighted sampling from the model pool.
%

\noindent
With the default reasoning + non-reasoning mix on the MMLU-Pro test set (2100 questions $\times$ 3 solvers = 6300 selections), Gemma is selected most often (1632) and Exaone least (547), giving a max/min ratio of 2.98$\times$.
%
In \autoref{fig:popularity2}a, y-axis represents population coefficient-of-variance for each model pool.
%
In all non-Reasonings (allnonR), the strongest remaining models dominate (Gemma 53\%, Qwen 24\%) while Llama and Granite each fall below 2\%, pushing max/min to 92.4$\times$.
%
\textbf{This proves that the popularity skew of solvers is sensitive to the pool composition.}

% Now  we combine the effect of popularity skew and varied token-budget of model classes when models are allocated in each GPU workers in round-robin fashion, in the order of first-seen solver for given test questions. In default case, Gemma+Exaone and Qwen got allocated in GPU 0 and GPU 2 which finishes a lot earlier where GPU 1 and GPU 3 are the stragglers which contributes the total expert inference time. Notice that for a mixed scenario, some workers stay idle for the longest time. Reasoning models generate 6–13× more tokens per prompt and combining with popularity skew, total active seconds for the two R1 workers (~2546–2620s) vs the others (~165–430s) — a ~6–16× imbalance. It is worth noting that for allR or allnonR cases as well the idle GPU time is significant. worker 0 of allR got two reasoning solvers (StratosR1+QwenR1) and spent 7039s active; worker 2 got one small reasoning solver and spent 2232s — a 3× wall-time spread from count-skew + token-skew acting together.

\autoref{fig:popularity2}b shows what happens when these skewed solver demands combine with token-budget disparity.
%
We consider a round-robin allocation (in first-seen-solver order in the available query queue), a scheme that commits each solver to a worker before any cost or count signal is observed.
%
In the default pool, reasoning workers dominate wall time: worker 1 (QwenR1+GLM, 2620s) and worker 3 (LlamaR1, 2546s) take 6-16$\times$ longer than worker 0 (Gemma+Exaone, 430s) and worker 2 (Qwen, 165s).
%
Notably, worker 0 (W0) holds the most popular solver (Gemma) in the entire pool, yet finishes earlier; because reasoning models generate 6-13$\times$ more tokens per prompt.
%
Per-prompt cost dominates popularity-count whenever the two solver classes mix.
%
The idle GPU time is also significant for allR and allnonR cases.
%
W0 of allR got two reasoning solvers (Stratos+QwenR1) and spent 7039s active; where W1 (DLER+OREAL) and W2 (LlamaR1) finishes 4$\times$ and 3.15$\times$ earlier respectively.
%
Each of W1 and W2 process same number of prompts (25.4\% and 25.1\%), but DLER prompt-cost being cheaper, it finishes faster.
%
No single factor explains the imbalance in GPU idling: a cost-aware scheduler must balance $\sum(\text{prompts} \times \text{per-prompt cost})$ per worker rather than either quantity alone.



% 2. Compare with data concurrency, major factors affecting
% a. visible load time if total generation time is less
% b. GPU underutilization for low shard size

% An alternate strategy to eliminate GPU idling time is to use data concurrency for each solver. In this strategy, a full copy of each solver is loaded in all 4 GPU workers, and the total queries that needs that solver is divided by the number of GPU workers and passed into. This way for each worker, it process similar number of queries and they finish in similar time. This goes on sequentially solver by solver on all GPUs. on a sidenote, tensor parallelism is not considered because we use 7B scale models which fits comfortably in a single A100 GPU, and allreduce operation of TP, make the overall runtime way worse. For roundrobin (each GPU worker has different solvers), each worker run their assigned solvers serially and the model load time overlap across workers, so `wall ≈ max_w(Σ_m load+gen)`, but they lose upto 45% of GPU-time to idle. In data concurrency, it loops solver-by-solver with a sync barrier between models, so the critical-path wall is `Σ_m max_w(load+gen)`, but it cuts the within-model straggler waste. In the figure, only in the allnonR case, data concurrency is worse than RR (do not use the term RR, it sounds too naive) because the small compute budget cannot amortize the replicated load.

\SM{Shorten this if kept here. Put rest in appendix and refer this to the beginning of the motivation. Later if we need more content we may need to move this in the same place}
\insertFigure{dp}{Overview figure.}
% \betterparagraph{III. The Pitfalls of Data Concurrency and Over-Sharding}
% % \SK{This is too detailed ... you need to make it precise and convert to 1/2 of current size.}
% An alternative to per-worker solver placement is data parallelism (DP). 
% %
% It loads a complete copy of each solver on all 4 GPUs, evenly shards the prompts requiring that solver, across workers, and processes solvers sequentially with a sync barrier between them.
% %
% The two strategies differ in critical path: solver-per-worker or round-robin placement runs each worker's assigned solvers serially with model loads overlapped across workers, giving $\text{expert\_latency} \approx \max_{w}(\sum_{m} \text{load} + \text{gen})$ and exposing within-worker stragglers as idle time.
% %
% DP serializes over models but parallelizes within each, giving $\text{expert\_latency} \approx \sum_{m} \max_{w}(\text{load} + \text{gen})$ and replacing straggler-idle with a replicated load tax (every model loaded on every worker).
% %
% \autoref{fig:dp}a confirms the tradeoff; DP cuts the \textasciitilde45\% idle share of roundrobin runtime to give a overall \textasciitilde9\% wall-time improvement in default model-pool, and similarly improves allR (7080s to 6431s).
% %
% In allnonR, however, DP is \textasciitilde29\% slower (631s vs 892s), the per-solver generate budget is too small to amortize serialized loads.

% Also in data concurrency throughput drops when it shards the same workload across 4 GPU workers. every solver's RR point sits at the right (large shard, near-peak throughput). The gap from RR to DP for that solver quantifies the lost throughput from over-sharding. vLLM uses continuous batching and the GPU only reaches peak throughput when there are enough in-flight prompts to keep the model fully busy. Below some threshold (depends on model architecture and GPU compute, memory), throughput scales sub-linearly with batch size, then the GPU starves. Above the threshold throughput flattens.
% Qwen / Exaone / GLM RR shards are above the threshold → high tok/s.
% Their DP shards (137-239) are below it → throughput collapses.
% Gemma's DP shard (408) is at/above the threshold → essentially no collapse. Gemma started with far more prompts than any other solver in default because recruit_agents over-picked it. So Gemma never enters the "small-batch under-utilization" regime that bites the others.
% Reasoning models cluster around 1000-2000 tok/s independent of shard size (explain if possible in short).
% Potentially if we can eliminate the idle GPU time RR type of scheduling will provide better overall latency and it also benefits from using the peak GPU throughput for higher prompt volume per solver.
% DP incurs a second cost due to throughput collapse from over-sharding.
% %
% vLLM\citep{kwon2023efficient} relies on continuous batching, which only reaches peak tok/s when enough prompts are in flight to keep the model fully utilized.
% %
% Below a model and GPU-dependent threshold, throughput scales sub-linearly with batch size, and at very small batches, the GPU starves.
% %
% \autoref{fig:dp}b makes this visible by plotting the throughput of each model in the default model-pool for both roundrobin (full data shard) and DP (1/4 shard).
% %
% The full-shard points sit at the right for each color (solver), showing peak-throughput.
% %
% The DP points are located on the left (137-239 prompts per shards) and throughput is reduced by 40-60\% for Qwen, Exaone, and GLM.
% %
% Gemma is an exception because skill-weighted recruitment over-picked it in the default pool, even its 1/4 shard (\textasciitilde408 prompts) stays above its saturation threshold. Thus, DP barely costs throughput for Gemma.
% %
% Reasoning models cluster around 1000-2000 tok/s, regardless of shard size.
% %
% Their long autoregressive decode phase is memory-bandwidth bound, so a handful of in-flight prompts already saturate HBM and additional batch yields little.
% %

% Taken together, DP trades off straggler-idle time for two new costs: serialized load and reduced throughput per shard.
% %
% It only wins when the per-solver generate budget is large enough to absorb both.
% %
% Solver-per-worker placement, by contrast, operates at peak per-shard throughput and pays the model load only once per worker.
% %
% Its sole weakness is idle time from popularity and cost-skew.
% %
% Next, we develop a scheduler that assigns cost-aware solvers to workers, balancing the load and closing idle gaps.

% \begin{table}[htbp]
%     \centering
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{lrrrrrrr}
%         \toprule
%         Mode & Wall (s) & LBE & Straggler & Generate (s) & Vis. Load (s) & Idle (s) & Idle \% \\
%         \midrule
%         dp\_allR & 6431 & 0.88 & 0.74 & 20482 & 286 & 3586 & 14.24\% \\
%         dp\_allnonR & 892 & 0.97 & 0.94 & 1392 & 340 & 284 & 9.50\% \\
%         dp\_default & 2442 & 0.93 & 0.88 & 6872 & 331 & 983 & 10.72\% \\
%         roundrobin\_allR & 7082 & 0.57 & 0.25 & 15797 & 91 & 12082 & 42.91\% \\
%         roundrobin\_allnonR & 632 & 0.57 & 0.29 & 1022 & 101 & 1029 & 43.42\% \\
%         roundrobin\_default & 2663 & 0.55 & 0.06 & 5492 & 104 & 4720 & 45.03\% \\
%         \bottomrule
%     \end{tabular}%
%     }
%     \caption{Add your caption here. \SK{Convert to plot. with the key numbers, not all numbers are needed..Name the first col in a more readable way, without `\_'}}
%     \label{tab:performance_comparison}
% \end{table}



==> Sections/05_CaseStudies.tex <==

\section{Case Studies}
\label{sec:case_studies}

\insertWideFigure{memory_footprint_6}{
% Memory footprint of the prefill stage for Transformer, SSM, and Hybrid models on the target platforms: (a) consumer GPU (RTX 4090) and (b) edge GPU (Jetson Nano Orin)
Memory footprint of prefill stage for Transformer, SSM, and Hybrid models on (a) consumer GPU (RTX 4090) and (b) edge GPU (Jetson Nano Orin)
% \HK{include y axis tick labels. It is currently hard to understand what the "2cm" of the bar means; is it 1GB? 2GB?}
% \HK{Let's remove reserved memory. I don't think this provides valuable insights, and the explanation given in the text is not quite clear; it will likely do more harms than goods.}
}
%Demonstrating the capability of SSMs to extend input context length beyond transformers can support, showing a distinct range where SSM can only operate. We conducted experiments on two platforms: (a) Consumer GPU (above) and, (b) embedded GPU, Jetson Nano Orin (below).}

%Some text on what we are going to discuss in this section and what specific case studies areas we are focusing on. 
% A thorough analysis for all categories of model considered in \autoref{tab:model_zoo} were performed in both the platforms stated in \autoref{tab:gpu_setup}. Some insightful results are explained below in forms of individual case studies. We focused on the usability of architecturally different type of models on extremely long context case in \ref{subsec:mem_footprint}. Following that, we performed extensive characterization experiments for different operator classes present in all sets of models we considered. Also, we showed the implications of deploying them in edge devices and a comparative analysis was performed. 
%This section presents a thorough performance analysis of models listed in \autoref{tab:model_zoo_short}, conducted on the consumer and edge platforms listed in \autoref{tab:gpu_setup}. 
%
% \TODO{intro the subsections of case studies}
We present performance analysis results with some highlighted cases that deliver new insights.
%
In \autoref{subsec:scalability_mem_footprint}, we investigate the memory footprint of the evaluated models and identify the maximum sequence length supported by each model on each evaluated platforms listed in~\autoref{tab:gpu_setup}.
%
We quantify the shift in energy consumption and end-to-end performance of all models in \autoref{subsec:energy_results}.
%
In \autoref{subsec:op_breakdown}, we perform an extensive performance characterization in the  operator granularity. %classes present in each model categories. 
%
Finally, we explore the performance implications of deploying these models on resource-constrained edge devices and provide a comparative analysis of the results.


% \subsection{Characterizing the ability to run long context models on constrained memory devices}
% \subsection{Characterizing Long-Context Memory Limits}
\subsection{Memory Footprint and Scaling Limits}
\label{subsec:scalability_mem_footprint}
%\subsubsection{Memory Footprint and Scaling Limits}
%\label{subsubsec:mem_footprint}

% prefill:
We present memory footprint characterization results over increasing sequence length in~\autoref{fig:memory_footprint_6}.
%
%We push the language models to their operational limits to characterize their memory footprint while processing very long-context input sequences on memory-constrained devices.
%
Our experiments focus on a single, long prefill stage to isolate the bottleneck in long-context applications (e.g., document summarization using RAG).
%
At the end of the prefill stage, memory pressure peaks because storing all prefill token activations ($S_{in}$) alongside the initial KV cache is required. 
%
In contrast, the decode stage processes tokens autoregressively, keeping only a single token’s activation in memory while the KV cache grows.
%
Reaching an OOM state during decode would require an excessively large number of output tokens ($S_{out}$).
%
%When the sequence length increases in the prefill-phase, the memory requirement of storing activation of all prefill tokens and the KV cache creates instantaneous memory pressure.
%
%In contrast, the memory pressure for activation in the decode stage is mitigated due to the nature of token-by-token generation.
%
%However, the KV cache keeps growing with the generated tokens.
%
Hence we scale the $S_{in}$ logarithmically from 1024 to 8192, then linearly in increments of 8192 up to 65536, and then in increments of 16384 until 180224.
%
We include additional data points at the end to capture behavior in some extreme cases.
%
We provide breakdowns into weight, activation, and KV cache (if applicable).
%
%The plotted data for a particular model extends along the sequence length axis only until the total memory footprint exceeds the device's physical memory capacity.
%
We stop plotting the data when we encounter the out-of-memory (OOM) issue.
%
For instance, the Phi-3-mini executes successfully at 4096 tokens but fails at 8192.
%
This indicates that its OOM threshold lies strictly between these two points.
%
%We show The 24GB memory capacity of the GPU is marked by a red horizontal line.
%
%Additionally, the dashed lines represent the total memory reserved by PyTorch, which is typically higher than the runtime requirement due to its conservative memory management.
%

From the Transformer category, we evaluated Qwen2.5 (0.5B), Llama3.2 (1B), and Phi-3-mini (3.82B).
%
While Phi-3 uses a classical decoder architecture, Qwen2.5 and Llama3.2 employ techniques like GQA and SwiGLU, which enhance scaling during inference.
%
On the consumer GPU (~\autoref{fig:memory_footprint_6}(a)), due to Phi-3's larger weight and KV cache size, Phi-3 was bottlenecked at a sequence length of 4096.
%
In contrast, Qwen and Llama extended much further, reaching 57,344 and 65,536 tokens, respectively.
%
For the SSMs, we considered Mamba and Mamba-2 (both \textasciitilde790M).
%
Although SSMs initially require higher memory footprint than Qwen, that of SSMs scales better with the lower activation memory growth and the absence of the KV cache.
%quickly demonstrated their long-context superiority through lower activation memory growth and the absence of a KV-cache.
%
Both Mamba and Mamba-2 are capable to handle up to 220K sequence length within the 24GB limit, which is unmatched by any similarly sized Transformer model.
%
This suggests that for contexts beyond \textasciitilde73K tokens, SSMs are the only viable architecture on consumer-grade GPUs without offloading.
%
We also benchmarked an earlier hybrid model Zamba2 (1.2B), which operated up to 49K tokens but showed significant KV cache consumption from its Transformer components due to not using GQA nor similar KV cache compression techniques.
%
% As hybrid architectures are still nascent, we expect future iterations will better bridge this long-context gap.
% \TODO{add falcon in the graph}
A recently released hybrid model Falcon-H1 bridges this gap and can perform inference until \textasciitilde164K, way beyond Transformer models can reach with matching accuracy performance.
%
%The activation memory for this model in the figure already includes the KV cache, as we could not capture it separately.
%

%We observe fluctuating reserved memory size in PyTorch (e.g., That of Mamaba-790M decreases for the sequence length of 147K).
%
%This originates from the PyTorch's conservative memory allocation behavior that initially reserve a large amount of memory and reduce it when the memory consumption is near 
%An interesting side-observation is PyTorch's memory allocation strategy; initially, it reserves a high memory slack, but as usage nears the hardware limit, it reduces this reserved buffer, causing occasional dips in the reserved memory plot even as usage increases.
%

\betterparagraph{Impact of Efficient inference-engines}To compare these intrinsic limits in highly optimized production environments, we integrated these models into our framework with vLLM (chunked prefill enabled).
%
The OOM frontier for the Transformer-based Qwen extends significantly, going beyond the \textasciitilde57K token limit observed in native PyTorch to ~81K tokens in vLLM.
%
However, the maximum sequence lengths for Mamba and Falcon-H1 remain unchanged for the vLLM-support being experimental.

\betterparagraph{Impact of Quantization} 
In this case study, quantized checkpoints were not used because the available pretrained weights of different model classes use diverse and often incompatible quantization schemes.
%
To show the impact of quantization on memory scaling, we evaluated Qwen2.5-0.5B using GPTQ, a one-shot weight-only quantization.
%
This approach reduced the weight size by 3.6$\times$ (from 942 MB to 260 MB) while preserving activation memory (including the KV cache) in BF16 to maintain accuracy.
%
Despite the weight compression, the maximum supported sequence length for Qwen only increased slightly (from \textasciitilde57k to \textasciitilde59k).
%
For SSMs, we evaluated the model using Quamba2\cite{chiang2025quamba2} weights (W4A8).
%
At a 57K sequence length, Quamba2 saves 1.65$\times$ (4324 MB down to 2613 MB) on the total memory footprint.
%
This reduction significantly extends its OOM frontier.
%
While quantized checkpoints for the specific hybrid models evaluated are currently unavailable, we expect similar scaling trends when equivalent activation and weight quantization techniques are applied across architectures.

%
For the edge GPU (~\autoref{fig:memory_footprint_6} (b)), we exclude Phi-3 model as even its weights alone could not be accommodated within the available memory.
%
The primary observations from this experiment align with those from the consumer GPU, except for the significantly reduced operating range for all models.
%
On this severely constrained platform, SSMs and hybrids once again demonstrated a clear advantage, proving capable of processing contexts greater than 16K tokens while the Transformers could not.
%
\textbf{Overall, SSMs can operate at a maximum sequence length that is up to 4$\times$ greater than what is achievable by the Transformer models.} %Also, Hybrid models may incorporate KV compression techniques like GQA to be competitive with SSMs in terms of scalability.}
% In this case study, we will push the language models to their limits for processing very long-context input sequences on memory constrained devices. First, from \autoref{fig:memory_footprint4}, it can be seen that models from all 3 categories are analyzed for the memory footprints during their forward pass on consumer class GPU. A wide range of sequence lengths were considered starting from 256 and doubling that each time, but for better visibility after 8192, a step size of 8192 was taken until 155648, and then few more sequence lengths were tried to handle the outlier cases. The maximum GPU memory available is defined with the red horizontal line (24GB in this case). The total memory footprint of the model is visually split within the model weights, activation memory consumption, and KV cache (if any). PyTorch, being conservative with respect to memory handling, always reserves a bit higher memory than the runtime requires, which is expressed with the dashed lines.
% From transformers category, Qwen2.5 (0.5B), Llama3.2 (1B) and Phi-3-mini (3.82B) were considered. While Phi-3 uses classical decoder-only architecture, Qwen2.5 and Llama3.2 uses techniques like Grouped-Query Attention (GQA), SwiGLU, RMSNorm for efficiency and it helps to scale the inference. Due to higher weight and KV cache size Phi-3 was bottlenecked at sequence length 4096, where Qwen and Llama could continue until 57344 and 65536 respectively. Even though the Llama model is double the size of Qwen model and Llama having a larger KV cache always, the prefill activation size of the former is lower than that of the later for a very large sequence length of 57344. For SSM models, mamba and mamba2 (both 790m) were considered. Even if initially the total memory footprint was higher than Qwen, soon with higher sequence lengths, SSMs showed lower activation memory and no KV-cache requirement. Both mamba and mamba2 could reach upto staggaringly high 220K sequence length within 24GB memory limit which is unachievable by any similarly sized transformer models by far. So on and above 73K sequence length range, SSM can only operate fitting inside a consumer grade GPU (without any offloading opportunities considered). We also benchmarked a hybrid model Zamba2(1.2B) which could operate until 49K, and it showed a higher KV cache consumption from its transformer counterpart. As the state of hybrid models are nascent, we expect in future, the hybrid models will bridge this gap of long-context inference viability with trading off the accuracy. Also, here one interesting observation is Pytorch being conservative at first keeps higher memory slack reserved for the runtime, after a point when that is not sufficient it cuts shorts the extra reserved memory. So sometimes we can see the dip in the reserved memory with increasing frequency.
% Next, we perform this experiment on Jetson platform \autoref{fig:memory_footprint4} ????(b), Phi3 was eliminated as the weight only was not being accomodated in the 8GB memory. The primary observations are matching with the last one only the operating range of sequence length of different categories of models are different. SSMs could operate >16K context when the others could not. 
% \insertWideFigurepng{memory_footprint2}{caption7}
% \insertWideFigurepng{memory_footprint4}{caption9}
% \insertWideFigurepng{memory_footprint2a}{caption8}


% generate:


% The state space model that emerged to solve language modeling tasks, needs some carefully written hardware-aware kernels to make it possible for real-time deployment. previous studies exist (cite nongemm bench paper) that thoroughly analyzes the distribution of GEMM and non-GEMM ops, also how the diversity of dominating operators are found across a large set of different models. In this subsection we will investigate on the effect of SSM specific operations like selective scan and causalconv1D under various deployment configurations including seq length, deployment platform etc. These operators can not be staraightforwardly classified as GEMM or non-GEMM operators as they have mix of both in finer granular level. For example operators like mambainnerfn  or mambasplitconv1dscancombinedfn often contains a diverse set of memory handling and linear transformation type of operations. But as a whole, as the SSM operators contribute to larger part of operational runtime, it makes more sense to consider them as a seperate category. Sometimes in the graphs the activation function (such as silu) operators are not visible because the SSM operators already includes those functions and accounting for their contribution. 

\subsection{Energy Consumption \& End-to-end Performance}
\label{subsec:energy_results}

\insertFigure{energy_throughput}{(a) Inference energy consumption and (b) end-to-end throughput performance of Qwen2.5-0.5B (Transformer), Mamba2-780m (SSM), and Falcon-H1-0.5B (Hybrid) over sequence length on RTX4090}
%Transformers are energy-efficient at short sequences, but becomes prohibitive at long contexts ($4\times$ higher than SSMs at 57k tokens)


\autoref{fig:energy_throughput}(a) presents the total energy consumption (in J) of the three models (Transformer, SSM, and Hybrid) when increasing sequence lengths from 1K to 57K.
%
Note that the Y-axis is presented in log scale to accommodate the wide range of the data.
%
In short contexts (<16K tokens), the Transformer model (Qwen2.5) consumes the least energy, benefiting from highly optimized GEMM kernels.
%
However, this trend sharply reverses as sequence length increases.
%
At 57K tokens, the quadratic computational burden of the Transformer results in high energy usage (1492 J), which is approximately \textbf{4$\times$} higher than the Mamba-2 SSM (370 J).
%
\textbf{The Hybrid Falcon-H1 model (613 J) effectively bridges this gap, offering a balanced profile that is 2.4$\times$ more energy-efficient than the Transformer} while retaining the accuracy gains discussed in \autoref{sec:background}.
%
% Considering the higher accuracy delivered by SSMs, the results imply that Hybrid models are promising options for efficient and effective long-context inference.
Hybrid models are promising options for efficient and effective long-context inference, given their higher accuracy compared to SSMs.

% \subsection{End-to-end Computational Performance}
% \label{subsec:e2e_performance}
We measure the overall throughput of text generation scenario (includes prefill and decode) across three model categories for different sequence lengths.
%
In our experiment, we consider batch sizes of 1 and 256 tokens as outputs.
%
Qwen outperforms in end-to-end performance with higher throughput in shorter sequences.
%
At 32K input sequence length when generating same output tokens, the TPOT jumps 2.4$\times$ more than the one in lower input sequence.
%
For SSM and Hybrids, TPOT remains fairly flat across experimented sequence lengths.
%
In \autoref{fig:energy_throughput}(b) \textbf{Mamba2 and Falcon-H1 attains 2.64$\times$ and 1.54$\times$ of the throughput of our baseline Transformer model at 32K sequence length}.

\subsection{Operator level performance}
\label{subsec:op_breakdown}
% State Space Models, which have emerged to solve long-context language modeling tasks, require carefully designed hardware-aware kernels to be viable for real-time deployment.
%
% Previous studies have thoroughly analyzed the latency distribution of General Matrix Multiplication (GEMM) and non-GEMM operations, highlighting the diversity of dominant operators across a large set of different models \cite{karami2025nongemmbenchunderstandingperformance}.
%
We investigate the performance implications of SSM-specific operations, such as \texttt{selective scan} and \texttt{causalconv1D}, under various deployment configurations, including sequence length changes and deployment platforms.
%
These novel operators cannot be straightforwardly classified as GEMM or non-GEMM.
%
At a finer granularity, they are composed of a mix of both types of operations.
%
For instance, low-level fused kernels like \texttt{mambainnerfn} or \texttt{mambasplitconv1dscancombinedfn} in popular SSM implementations often contain a diverse set of memory handling, element-wise arithmetic, and linear transformation operations.
%
Since these fused SSM operators contribute to the majority of the model's running time, it is more practical to analyze them as a separate, distinct category.
%
% It is also important to note that in the subsequent performance breakdown graphs, common activation functions like \textit{SiLU} may not be explicitly visible.
Some common activation functions like \textit{SiLU} are not be explicitly visible in the subsequent performance breakdown graphs due to its minor contribution to the total latency and/or operator fusion.
%
In this study, we focus on SSM and hybrid models as the bottlenecks of Transformers are well-studied~\cite{karami2025nongemmbenchunderstandingperformance}.


\insertFigure{mamba_breakdown_2a_singlecol}{Latency breakdown of SSMs into operator classes targeting RTX GPU on (a) the first generation of 130m mamba model and (b) second generation of the same family of model}
% \insertWideFigure{hybrid_breakdown_2a}{Operator-wise latency breakdown for Hybrid models on consumer GPU. (a) Zamba2 model with 1.2B params, (b) Hymba model with 1.5B params on the right. (c) Latency breakdown results for Mamba-130m model in an edge platform (Jetson Nano Orin)}



\subsubsection{SSMs on Consumer GPU}
\label{subsubsec:ssm_on_consumer}
To further understand model-specific characteristics, we analyze the operator-level latency breakdown of the state-of-the-art Mamba and Mamba-2 models as sequence length increases on the consumer-GPU, with results presented in \autoref{fig:mamba_breakdown_2a_singlecol}.
%
% The experiments are conducted on the consumer-grade GPU detailed in Table~\ref{tab:gpu_setup}. 
%
%By increasing the input sequence length from 256 to 131,072 tokens (doubling in each step), we specifically focus on the computationally intensive \textit{prefill} phase.
The input sequence length is increased logarithmically from 256 to 131072 tokens.
%
Each bar in the figure illustrates the percentage of total latency contributed by different operator categories.
%
The \textit{SSM-specific operators} are at the bottom, followed by \textit{GEMM-based operators}, and finally the \textit{non-GEMM operators}, which are sorted from highest to lowest contribution.
%

For the Mamba model, we observe a clear trend: as the sequence length grows, the relative latency of non-GEMM operators—such as normalization, memory, and arithmetic operations—steadily decreases.
%
Conversely, the contribution from GEMM operations (e.g., \texttt{matmul}, \texttt{linear}) monotonically increases, indicating that the workload becomes more compute-bound at longer sequences.
%
However, the latency share of the core SSM operators remains relatively flat.
%, showing only a marginal dip before rising slightly at sequences longer than 8192 tokens.
%
% You can strengthen this by adding a sentence or two of why it might be happening. For example, when the SSM operator's contribution dips and then recovers, could this be due to a shift in which sub-operation becomes the bottleneck (e.g., moving from being memory-bound to compute-bound) as caches are filled? Adding such hypotheses makes the analysis more insightful.

When examining the newer Mamba-2 model under the same conditions, we observe similar trends.
%
However, the core SSM operator in Mamba-2 (\texttt{mambasplitconv1dscancombinedfn}) accounts for a larger portion of the total latency compared to its Mamba-1 counterpart (\texttt{mambainnerfn}).
%
This is due to architectural advancements in Mamba-2, which supports much larger state dimensions (from 16 to 64 or higher), leading to a more computationally intensive selective scan operation.
%
Furthermore, a key distinction emerges within the non-GEMM category: for Mamba-1 memory operators (transpose, slice, reshape etc.) are the dominant amongst non-GEMM component after normalization.
%
In contrast for Mamba-2, arithmetic operators consistently contribute more to the latency than memory ops.
%
This also can be attributed to Mamba-2's introduction of increased state-dimension and the multi-head structure, which expands the head dimension (e.g., from 1 to 64) compared to the earlier architecture.
%
%However, a key distinction emerges within the non-GEMM category: for Mamba-2, arithmetic operators consistently contribute more to the latency than memory-related operators.
%
%We attribute this to Mamba-2's introduction of a multi-head structure, which expands both the head dimension (e.g., from 1 to 64) and the state dimension compared to the earlier architecture.
% \TODO{has this been repeated earlier?}
%
%These changes raise the computational cost of state updates relative to pure data movement.
%
%This contrasts with Mamba-1, where memory operators (transpose, slice, reshape etc.) were the dominant amongst non-GEMM component after normalization.
%
%Furthermore, the core SSM operator in Mamba-2 (\texttt{mambasplitconv1dscancombinedfn}) accounts for a larger portion of the total latency compared to its Mamba-1 counterpart (\texttt{mambainnerfn}).
%
%This also can be attributed to architectural advancements in Mamba-2, which supports much larger state dimensions (from 16 to 64 or higher), leading to a more computationally intensive selective scan operation.
%

Overall, we find that the performance of SSMs are dominated by newer SSM-specific operators, unlike Transformers that are usually dominated by GEMM or non-GEMM counterparts.
%
\textbf{This implies that optimizing SSM-specific operators is crucial for SSM performance for long context.}




% We analyze the operatorwise latency breakdown of state-of-the-art SSMs (in percentage) with increasing sequence length in \autoref{fig:mamba_130m_breakdown}. The experiments are performed on the consumer level GPU mentioned in \ref{tab:tab_hw} and sequence length increase is happening for input sequence,  hence the scenario we are discussing in prefill (compute bound). The sequence length tried ranges from 256 to 131072 with doubling in every step. The SSM specific operators are shown in the bottom of each bar, then above it GEMM operator's contribution, above it are the non-GEMM operators sorted from highest to lowest contribution (bottom to top). 

% For the smallest mamba model (130m parameter), with increasing sequence length, the contribution of non-GEMM operators (such as normalization, memory related ops, arithmetic ops) keeps reducing. On the other hand the GEMM operations (e.g. matmul, linear) monotonically increases its contribution with increasing sequence length. Surprisingly, The contribution of SSM operators drops marginally in the beginning but rises slightly after seq length 8192. Overall, it remains flat. 
% Now when we look at the newer mamba2 (130m) with the same experimental setup, we notice the similar characteristic observations. Difference with mamba model is for every sequence arithmetic operators contribute more than memory related operators. For mamba memory operators were always contributing majorly among the non-GEMM operators (just after normalization). Compared to Mamba-1, Mamba-2 allows much larger state dimensions (from N=16 in Mamba-1 to N=64 to N=256 or even higher in Mamba-2). This can explain the larger share of SSM based operator (mambasplitconv1dscancombinedfn) in mamba 2 than the one in mamba (mambainnerfn)

% \insertFigurepng{zamba2_op_breakdown}{caption4}
% \insertFigurepng{hymba_op_breakdown}{caption3}

% \betterparagraph{Hybrid Models}
% We will be shortly discussing how the op distribution looks like for Hybrid models, Zamba2 (1.2B) and Hymba(1.5B). The results are presented in \ref{}. Similar test environments were taken and doubling sequence length were performed until out of GPU memory error is reached. In these cases, the models were taken from huggingface hub. It is important to notice that cudastreamsync is often present in different positions of the model graph, so in those time the CPU can not proceed with the next operation until the last operation's GPU counterpart is not completed. So these might attribute to longer contributions in specific operations, we are reporting the CPU and GPU value combined for each type of operators. Unique observations are found for individual hybrid models. For Zamba2 all non GEMM operato   rs contibutes to lesser time with increasing sequence length except the arithmetic operations. However, the contribution of SSM operator reduces and GEMM stays in the similar range. On the other hand, Hymba \ref{} has significant part in non-GEMM that is torch pre-compiled. All the other operators in Hymba shows diverse variability. One major observation is that it spends a lot of time in memory operations in high sequence length.

\insertFigure{hybrid_breakdown_2a_singlecol}{Operator-wise latency breakdown for Hybrid models on consumer GPU targeting (a) Zamba2(1.2B params) and (b) Hymba (1.5B params).}
\subsubsection{Hybrid Models on Consumer GPU}
\label{subsubsec:hybrid_on_consumer}
We evaluate the latency breakdown into operators in hybrid models: Zamba2 (1.2B) and Hymba (1.5B)% \TODO{if time permits analyze Falcon}
, and present the results in \autoref{fig:hybrid_breakdown_2a_singlecol}.
%
The experimental setup remains consistent with our previous tests.
%
The input sequence length was doubled in each run until the consumer GPU ran out of memory.
%
%It is important to note that profiling these models often reveals \texttt{cudaStreamSynchronize} calls (not specific to the hybrid models) within the execution graph.
Profiling these models often uncovers \texttt{cudaStreamSynchronize} calls (not unique to the hybrid models) present in the execution graph.
%
In hybrid models, these synchronizations are often artifacts of sub-optimal implementations.
%
For instance, in Zamba2, functions like \texttt{torch.is\_nonzero} return boolean values that require an explicit memory copy from the GPU to the CPU, which inherently triggers the synchronization bottleneck.
%
These synchronization points force the CPU to wait for GPU execution to complete, which can artificially inflate the reported latencies of certain operators.
%
%Profiling these models often uncovers \texttt{cudaStreamSynchronize} calls (not unique to the hybrid models) present in the execution graph.
%
%These synchronization points force the CPU to wait for GPU execution to complete, which can inflate the reported latencies of certain operators.
%
The performance data we report combines both CPU and GPU time for each operator to provide a holistic view.
%

Our analysis reveals unique performance profiles for each hybrid model.
%
Zamba2 is built with Mamba2 backbone, so it is interesting to observe that the order of contribution of different operators in sub-categories is similar.
%
It uses full attention at shared layers without GQA or cross-layer cache sharing, resulting in notable KV cache pressure (leading to OOMs earlier, as seen in \autoref{fig:memory_footprint_6}(a)).
%
In contrast, Falcon-H1 utilizes a Mamba2 backbone with optimized attention that reduces KV cache, enabling longer sequences.
%
Hymba employs cross-layer KV cache sharing between consecutive layers and GQA within each layer.
%
This introduces additional memory copy and reference operations, which become visible as a pronounced bottleneck at high sequence lengths in \autoref{fig:hybrid_breakdown_2a_singlecol}(b).
%
It reveals an optimization potential in long-context scenarios for Hymba.
%
Furthermore, hybrid models often introduce context-switching overheads on the Streaming Multiprocessors (SMs), as the scheduler must alternate between compute-dense GEMM operations and memory-dense SSM warps, potentially disrupting pipeline efficiency.

% Zamba2 is built with Mamba2 backbone, so it is interesting to observe that the order of contribution of different operators in sub-categories is similar.
%
%As the sequence length increases, the relative latency of most non-GEMM operators decreases, with the notable exception of arithmetic operations.
%
%Concurrently, the contribution from the core SSM operator diminishes, while the share of GEMM operations remains relatively constant.
%
%In contrast, for Hymba a significant portion of its non-GEMM latency is attributed to a pre-compiled kernel from \texttt{TorchInductor}, while other operators exhibit less predictable trends. 
%
%A key observation for Hymba is that memory operations become a pronounced bottleneck at very high sequence lengths, highlighting a potential area for optimization in long-context scenarios.
% Notably, memory operations become a bottleneck at high sequence lengths, suggesting optimization potential in long-context scenarios.
%
\textbf{Unlike SSMs, Hybrid models' operation breakdown is not dominated by SSM-operators, but show variability related to rest of its architecture.}
%
This indicates that Hybrid models need careful characterization of performance to identify model-specific bottleneck, which our framework can assist.
%As we move towards pareto-optimal hybrid architectures, our framework will help visualize critical performance bottlenecks to unlock optimization opportunities.


\insertWideFigure{device_comparison_6}{(a) Latency breakdown results for Mamba-130m model in an edge GPU (Jetson Nano Orin), (b) Operator classes runtime breakdown comparison in two target platforms: Consumer GPU (left) and edge-GPU (right) for sequence length 1024}
%Comparative analysis of the contributions of different operator classes in two different deployment target platforms: Consumer GPU (left) and edge-GPU (right) for sequence length 1024

% \subsubsection{Edge deployment related observations and implications}

\subsubsection{SSM on Edge GPU}
\label{subsec:ssm_on_edge}
Edge platforms present numerous constraints, including limited memory size and bandwidth and weak compute capability.
%
To investigate impact of such limitations, we deploy Mamba on a Nvidia Jetson Orin Nano listed in~\autoref{tab:gpu_setup}, pushing the input sequence length to its maximum supported limit while maintaining the same deployment scenario used for the consumer GPU.
%
We present the results in \autoref{fig:device_comparison_6}(a).
%
While the achievable sequence length on the edge GPU is smaller than that on the consumer GPU, the overall trends in operator-wise latency contribution are broadly similar, as shown in \autoref{fig:mamba_breakdown_2a_singlecol}.
%
The core SSM operator's relative contribution remains nearly flat.
%
One unique observation is that the SSM operators' latency share for mamba is consistently higher on the Jetson platform, accounting for over 55\% of the total runtime across all tested sequence lengths, which \textbf{imply the increased importance of optimizing SSM operators in some SSMs on edge platforms.}

However, we also observe that the significance of SSM operators change over model generations. 
%
For Mamba-2, SSM accounts for smaller latency share on the edge GPU than that on the consumer GPU.
%
However, the trend is opposite for the original Mamba.
%
Despite this shifting internal balance, the combined contribution of SSM and GEMM operators remains the dominant portion of the workload on both devices, consistently accounting for over \textbf{75-80\%} of the runtime.
%
This indicates that \textbf{significant optimization opportunities still exist within the core SSM operators} of such vanilla SSM architectures.

\subsubsection{Hybrid Models on Edge GPU}
\label{subsubsec:hybrid_on_edge}

As ~\autoref{fig:device_comparison_6} (b) presents that arithmetic and normalization operators become slightly more dominant while SSM operators become less significant compared to the consumer GPU case for Zamba 2. 
%
Hymba also presents overall similar trends as Zamba 2, while the significance of SSM operators increase, unlike Zamba 2.
%
Like the hybrid model on consumer edge GPU case, the results indicate that the performance bottleneck is model specific, and careful performance characterization is required for hybrids.

\subsubsection{Impact of Deployment Platforms}

We explore the performance impact from the choice of target platforms.
%
We deploy each evaluated model on both the consumer and the edge platforms with a fixed sequence length and present the detailed operator breakdown in \autoref{fig:device_comparison_6}(b).
%
For Transformers, the edge device requires more absolute time to complete individual GEMM operations due to its lower peak throughput.
% , as shown in \TODO{refer to the raw latency figure}
%
However, when viewed holistically, the percentage of total runtime attributed to GEMM operations consistently declines across all Transformer-based models when deployed on the edge.
%
The counter-intuitive result is due to the \textbf{performance penalty for non-GEMM operators is more severe on the edge platform, causing their relative contribution to increase significantly}.
%
The specific non-GEMM bottleneck varies by model; for example, the dominant non-GEMM operator in Qwen is \textit{Normalization}, whereas for GPT-Neo, it is \textit{Memory}-related operations.
%
This underscores that optimizing non-GEMM operations is still a critical challenge for deploying Transformer models on edge devices.

For SSMs, as we discussed in~\autoref{subsubsec:ssm_on_consumer} and ~\autoref{subsec:ssm_on_edge},  we observe considerably different breakdown across two generations of the Mamba model family across platforms, while keeping SSM operators as the most dominant part.
%
We observe the similar trend across evaluated platforms, which indicate that \textbf{SSM operator is the prime optimization target regardless of the target platform}.


For hybrid models, as we discussed in~\autoref{subsubsec:hybrid_on_consumer} and~\autoref{subsubsec:hybrid_on_edge}, the performance profiles of recent hybrid models on different devices are  heavily model dependent, which requires target model-aware optimization.
%
We do not observe considerably different trend across deployment platforms, which implies that \textbf{optimization on one platform would benefit the performance on the other platform}.



% We tried deploying models from all the categories (Transformers, SSM and Hybrid) we are considering in this study and compared their runtime behaviour for a fixed sequence length for two different class of devices \autoref{fig:device_comparison}. (a) From the profiling trace information it was evident that, as the edge device has lesser peak throughput for GEMM operations it was spending more time in completing the same operation. But when we holistically visualize the contribution of GEMM operation it declines across all transformer based models on the edge device. The reason can be attributed to spending more time in non-GEMM operators, this also varies model to model. For example, major nonGEMM operator for Qwen is normalization whereas for GPT-neo it is memory related ops. Optimizing the non-GEMM operations in edge deployment scenario is more critical. (b) Two generations of State space model from the same family shows different trend of SSM operator share when we change the deployment device. For mamba2, Jetson spends less time in SSM, whereas for mamba it is the opposite. Overall if we combine SSM and GEMM it contributes to more than 75 to 80 percent of overall runtime in any of the devices. So, there are optimization opportunities in SSM based operators in vanilla SSMs. (c) The hybrid models have recently emerged and architecturally they have much diversity. NVIDIA chose to use Mamba as the SSM heads in their primary Hymba model (Hymba 1.5B) because it generally yielded lower training loss and better performance in hybrid models, which aligns with findings from other hybrid models like Jamba-1.5. Possibly due to that reason, the operator breakdown for hymba follows the mamba trend for the SSM operators. On the other hand, Zamba2 is based on mamba2 backbone, so its SSM operator contribution trend aligns with that of mamba2 in different deployment platforms.



% <maybe just add the parameter scaling dependent op  distribution point add here in short.????>





==> Sections/06_RelatedWorks.tex <==
\section{Related Works}
\label{sec:related_works}


==> Tables/tab_alias.tex <==
\begin{center}
\begin{table}
\caption{\bench Model aliases used in ~\autoref{fig:server_op_breakdown} and ~\autoref{fig:workstation_op_breakdown}.}
\scriptsize
\centering
\begin{tabular} {  | c | c | c |  } 

\hline
%
 \textbf{ Models }  & \textbf{Batch Size} & \textbf{ Model Alias }     \\
\hline
%
 \multirow{2}{*}{ViT Base 16} & 1 &  Vt-b b-1 \\ 
\cline{2-3} 
% 
 & 8 & Vt-b b-8  \\ 
\cline{1-3} 
%
\multirow{2}{*}{ViT large 16} & 1 & Vt-l b-1 \\ 
\cline{2-3}
%
& 8 &Vt-l b-8 \\ 
\cline{1-3}
% 
 \multirow{2}{*}{Swin Transformer tiny} & 1 & Sw-t b-1 \\ 
\cline{2-3}
%
& 8 & Sw-t b-8 \\ 
\cline {1-3}
% 
 \multirow{2}{*}{Swin Transformer small} & 1 & Sw-s b-1 \\ 
\cline{2-3}
% 
& 8 & Sw-s b-8  \\
\cline{1-3}
% 
 \multirow{2}{*}{Swin Transformer base} & 1 & Sw-b b-1 \\ 
\cline{2-3}
% 
& 8 & Sw-b b-8 \\
\hline
%
 \multirow{3}{*}{FasterRCNN} & 1 & FRCNN b-1 \\ 
\cline{2-3}
%
& 2 & FRCNN b-2 \\
\cline {2-3}
%
& 8 & FRCNN b-8 \\
\cline {1-3}
%
 \multirow{3}{*}{MaskRCNN} & 1 & MRCNN b-1 \\
\cline{2-3}
%
& 2 & MRCNN b-2 \\ 
\cline {2-3}
% 
& 8 & MRCNN b-8 \\ 
\cline {1-3}
% 
DETR & 2 & DETR b-2 \\ 
\hline 
%
 \multirow{2}{*}{GPT2} & 1 & gpt2 b-1\\
\cline{2-3}
%
& 64 & gpt2 b-64 \\ 
\cline {1-3}
%
 \multirow{2}{*}{GPT2 Large} & 1 & gpt2-L b-1 \\
\cline{2-3}
%
& 64 & gpt2-L b-64\\
\cline{1-3}
%
GPT2 X-Large & 1 & GPT2-XL b-1 \\
\cline{1-3}
%
 Llama2-7B & 1 & Llama2-7b b-1 \\
\cline {1-3}
%
\multirow{2}{*} {Bert} & 1 & bert b-1 \\
\cline {2-3}
%
& 64 & bert b-64 \\ 
\hline

\end{tabular}
\label{tab:alias}

\end{table}
\end{center}

==> Tables/tab_comparison_related_works.tex <==
\begin{table}
\caption{Comparing \bench with existing benchmarks: MLPerf~\cite{reddi2020mlperf}, LongTail Bench~\cite{longtailbench}, TorchBench~\cite{hao2023torchbench}, and \bench (This work).}
\scriptsize
\centering
\begin{tabular} {| c| c | c | c | c |  }
\hline

% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Benchmark  \\  
% \end{tabular}} 
% & 
% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Latency  \\ Breakdown 
% \end{tabular}} 
% & 
% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Popularity  \\ Driven 
% \end{tabular}} 
% & 
% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Micro-  \\Benchmark  
% \end{tabular}} 
% & 
% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Real Dataset  \\  Driven
% \end{tabular}} 
% & 
% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Plug Model  \\ \& Profile\\ 
% \end{tabular}} 

% \\
% \hline 

% MLPerf ~\cite{reddi2020mlperf} &  & & & \checkmark & \\
% \hline

% LongTail ~\cite{longtailbench} & & & \checkmark & & \\ 
% \hline

% TorchBench ~\cite {hao2023torchbench} & &  \checkmark & & \checkmark & \\
% \hline 
% \bench & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
% \hline

%Benchmark & Latency Breakdown & Popularity Driven & Microbenchmark & Real dataset driven & Plug model and profile \\

\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\textbf{Benchamrk}
\end{tabular}}
& 
\multirow{2}{*}{MLPerf}  
&  
\multirow{2}{*}{LongTailBench}
&
\multirow{2}{*}{TorchBench}
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
NonGEMMBench \\ (This work)
\end{tabular}}\\

&&&&\\


\hline 
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Real Usage  \\ Driven 
\end{tabular}} 
& & &
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\checkmark
\end{tabular}} &
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\checkmark
\end{tabular}}
\\
&&&&
\\
\hline
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Non-GEMM \\ Focused  
\end{tabular}} 
&& \multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\checkmark
\end{tabular}} &&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\checkmark
\end{tabular}} \\

&&&&

\\
\hline
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Real Dataset  \\  Driven
\end{tabular}} 
& \multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\checkmark
\end{tabular}} &&&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\checkmark
\end{tabular}}\\
&&&&
\\

\hline 

\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Plug Model  \\ \& Profile\\ 
\end{tabular}} 
& &&&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\checkmark
\end{tabular}}\\
&&&&\\
\hline
\end{tabular}
\label{tab:comparison_related_works}
\end{table}


==> Tables/tab_cpu_gpu_breakdown.tex <==
\begin{center}
\begin{table}
\caption{Breakdown of the execution time of operators for a selected models running on workstation platform. }
    \tiny 
    \begin{tabular}{|l|l|l|l|l|l|}
    \hline
        \multirow{2}{*}{Model}  & \multirow{2}{*}{Operator} & \multicolumn{3}{c|}{GPU + CPU} & CPU Only  \\ \cline{3-6}
        
        ~ & ~ & CPU Time  (us) & GPU time (us) & Total (us) & Total (us) \\ \hline
        
        \multirow{6}{*}{ViT-b16-batch-1} & GEMM & 16650.44227 & 2118.434442 & 18768.87671 & 42016.1409 \\ \cline{2-6}
        
        ~ & Non-GEMM  & 23768.86693 & 157.2054795 & 23926.07241 & 12514.59883 \\ \cline{2-6}
        
        ~ & Norm & 8699.684932 & 83.01369863 & 8782.69863 & 3347.78865 \\ \cline{2-6}
        
        ~ & Act & 3631.97456 & 25.23287671 & 3657.207436 & 1378.082192 \\ \cline{2-6}
        
        ~ & Arith & 8387.129159 & 44.95107632 & 8432.080235 & 4738.761252 \\ \cline{2-6}
        
        ~ & MemOp & 470.8493151 & 4.007827789 & 474.8571429 & 285.702544 \\ \hline
        
        \multirow{6}{*}{ViT-b16-batch-8} & GEMM & 16611.30159 & 8103.539683 & 24714.84127 & 244985.4127 \\ \cline{2-6}
        
        ~ & NonGEMM & 23351.06349 & 564.7619048 & 23915.8254 & 21208.52381 \\ \cline{2-6}
        
        ~ & Norm & 8555.555556 & 177.968254 & 8733.52381 & 4413.396825 \\ \cline{2-6}
        
        ~ & Act & 3583.174603 & 254.8571429 & 3838.031746 & 6105.063492 \\ \cline{2-6}
        
        ~ & Arith & 8232.777778 & 112.9365079 & 8345.714286 & 6596.142857 \\ \cline{2-6}
        
        ~ & MemOp & 533.984127 & 19 & 552.984127 & 353.984127 \\ \hline
        
        \multirow{7}{*}{Swin-small-batch-1} & GEMM & 39907.95499 & 2562.344423 & 42470.29941 & 62790.23092 \\ \cline{2-6}
        
        ~ & NonGEMM & 56343.23483 & 449.7377691 & 56792.9726 & 20763.49902 \\ \cline{2-6}
        
        ~ & Norm & 18493.18395 & 179.2328767 & 18672.41683 & 3384.569472 \\ \cline{2-6}
       
        ~ & Act & 7567.876712 & 50.15264188 & 7618.029354 & 2349.882583 \\ \cline{2-6}
        
        ~ & Arith & 15319.20548 & 55.95107632 & 15375.15656 & 6976.322896 \\ \cline{2-6}
        
        ~ & MemOp & 10762.09198 & 159.3933464 & 10921.48532 & 5138.966732 \\ \cline{2-6}
        
        ~ & Pooling & 404.1643836 & 5.007827789 & 409.1722114 & 179.6438356 \\ \hline
        
        \multirow{7}{*}{Swin-small-batch-8} & GEMM & 38748.79365 & 7742.52381 & 46491.31746 & 301921.3333 \\ \cline{2-6}
        
        ~ & NonGEMM & 54719.14286 & 1056.349206 & 55775.49206 & 35682.7619 \\ \cline{2-6}
        
        ~ & Norm & 18470.36508 & 453.6349206 & 18924 & 6848.746032 \\ \cline{2-6}
        
        ~ & Act & 7505.984127 & 220.9206349 & 7726.904762 & 8390.968254 \\ \cline{2-6}
        
        ~ & Arith & 15197.44444 & 194.5555556 & 15392 & 10655.71429 \\ \cline{2-6}
        
        ~ & MemOp & 10490.50794 & 182.1111111 & 10672.61905 & 6367.301587 \\ \cline{2-6}
        
        ~ & Pooling & 340.4444444 & 5.126984127 & 345.5714286 & 187.5714286 \\ \hline
        
        \multirow{7}{*}{GPT2-batch-1} & GEMM & 31184.20352 & 1224.491194 & 32408.69472 & 33756.36791 \\ \cline{2-6}
        
        ~ & NonGEMM & 98842.03131 & 433.5048924 & 99275.5362 & 35683.49511 \\ \cline{2-6}
        
        ~ & Norm & 8736.489237 & 78.7964775 & 8815.285714 & 1906.369863 \\ \cline{2-6}
        
        ~ & Act & 30429.26419 & 165.4657534 & 30594.72994 & 5303.311155 \\ \cline{2-6}
        
        ~ & Arith & 18503.88258 & 84.38551859 & 18588.2681 & 5178.23092 \\ \cline{2-6}
        
        ~ & MemOp & 24863.66928 & 66.57925636 & 24930.24853 & 10191.07632 \\ \cline{2-6}
        
        ~ & Softmax & 3940.872798 & 31.39921722 & 3972.272016 & 1072.44227 \\ \hline
        
        \multirow{7}{*}{GPT2-batch-16} & GEMM & 31957.41935 & 19423.06452 & 51380.48387 & 674009.7742 \\ \cline{2-6}
        
        ~ & NonGEMM & 97856.96774 & 17246.03226 & 115103 & 376959.0323 \\ \cline{2-6}
        
        ~ & Norm & 8719.193548 & 330.6774194 & 9049.870968 & 8241.451613 \\ \cline{2-6}
        
        ~ & Act & 30523.67742 & 10668.45161 & 41192.12903 & 207763.7097 \\ \cline{2-6}
        
        ~ & Arith & 18477.12903 & 3472.677419 & 21949.80645 & 71270 \\ \cline{2-6}
        
        ~ & MemOp & 24327.74194 & 1283.258065 & 25611 & 45067.12903 \\ \cline{2-6}
        
        ~ & Softmax & 3852.354839 & 1466.774194 & 5319.129032 & 31275.74194 \\ \hline
        
        \multirow{7}{*}{GPT2-Large-batch-1} & GEMM & 95700.28571 & 7637.911937 & 103338.1977 & 218225.3268 \\ \cline{2-6}
        
        ~ & NonGEMM & 302483.9648 & 1536.931507 & 304020.8963 & 132494.407 \\ \cline{2-6}
        
        ~ & Norm & 26186.90802 & 270.9549902 & 26457.86301 & 9476.976517 \\ \cline{2-6}
        
        ~ & Act & 92491.7319 & 628.0998043 & 93119.8317 & 25988.68297 \\ \cline{2-6}
        
        ~ & Arith & 57705.94521 & 303.6634051 & 58009.60861 & 25796.62622 \\ \cline{2-6}
        
        ~ & MemOp & 76773.90215 & 217.741683 & 76991.64384 & 34278.5362 \\ \cline{2-6}
        
        ~ & Softmax & 11540.80822 & 108.9471624 & 11649.75538 & 3886.178082 \\ \hline
        
        \multirow{7}{*}{GPT2-Large-batch-64} & GEMM & 101309.2258 & 139389.2581 & 240698.4839 & 5132246.935 \\ \cline{2-6}
        
        ~ & NonGEMM & 326921.6452 & 96818.35484 & 423740 & 1843876.968 \\ \cline{2-6}
        
        ~ & Norm & 26886.09677 & 1413.806452 & 28299.90323 & 44316.90323 \\ \cline{2-6}
        
        ~ & Act & 97057.64516 & 61441.77419 & 158499.4194 & 1043040.839 \\ \cline{2-6}
        
        ~ & Arith & 60932.19355 & 18790.06452 & 79722.25806 & 355737.3226 \\ \cline{2-6}
        
        ~ & MemOp & 86503.41935 & 6996.096774 & 93499.51613 & 201767.129 \\ \cline{2-6}
        
        ~ & Softmax & 12168.09677 & 8134.677419 & 20302.77419 & 156385.1613 \\ \hline
    
    \end{tabular}
    \label{tab:cpu_gpu_breakdown}    
\end{table}
\end{center}

==> Tables/tab_energy.tex <==
\begin{center}
\begin{table}
\caption{Most time-consuming non-GEMM operator groups for selected Models (Platform A, with GPU acceleration, average across batch sizes).}

\scriptsize
\centering

\begin{tabular} {   | c | c | c | c |  } 
\hline


\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Task \\ Domain
\end{tabular}} 
&
\multirow{2}{*}{
Model}
& 

\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Batch  \\ Size  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Energy \\ (J)  
\end{tabular}} 
\\

&&& \\

% \textbf{ Application } & \textbf{ Models } & \textbf{Batch} & \textbf{ Operator Group } & \textbf{\% of Exec.} 
%
%  &   &  \textbf{Size}& \textbf{Group }   & \textbf{Time }  \\
\hline
%
\multirow{12}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Image  \\ Classification
\end{tabular}}
}
% 
& \multirow{2}{*}{
 Vt-b} &  1  & 2.3 \\ 
\cline{3-4}
 & &  8  & 2.6 \\ 
\cline{2-4}


% 
& \multirow{2}{*}
{Vt-l} & 1  & 2.5 \\ 
\cline{3-4}
 & &  8  & 6.7 \\ 
\cline{2-4}

%
& \multirow{2}{*}
{Vt-h}  & 1  & 4.4  \\ 
\cline{3-4}
& & 8  & 12.1 \\ 
\cline{2-4}
% 
& \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Sw-t  
\end{tabular}}} & 1 & 1.9 \\ 
\cline{3-4}
& & 8  & 2.6 \\ 
\cline{2-4}

% 
&\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Sw-s  
\end{tabular}}} & 1 & 3.6 \\ 
\cline{3-4}
% 
& &  8 & 4.8 \\ 
\cline{2-4}
% 

&\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
Sw-b   
\end{tabular}}}  & 1 & 3.9 \\ 
\cline{3-4}
& &  8 & 5.5 \\ 
\hline
% 
\multirow{6}{*}{Object Detection} 
&  \multirow{2}{*}{FRCNN}
& 1 & 3.5 \\ 
\cline{3-4}
%
& & 1 & 19.4 \\ 
\cline{2-4}
% 
&  \multirow{2}{*}{MRCNN}  & 1 & 3.6\\
\cline{3-4}
% 
& & 1 & 19.6\\
\cline{2-4}
% 

& \multirow{2}{*}{DETR} & 1 & 5.8 \\ 
\cline{3-4}
& & 8 & 23.1 \\ 
\hline
% 
\multirow{4}{*}{Image Segmenation} 
&  \multirow{2}{*}{MF}
& 1 & 11.4 \\ 
\cline{3-4}
%
& & 8 & 40.6 \\ 
\cline{2-4}
% 
&  \multirow{2}{*}{Seg}  & 1 & 1.7\\
\cline{3-4}
%
& & 8 & 4.6 \\ 
\hline
% 
\multirow{8}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 NLP \\  
\end{tabular}}} 
& \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
gpt2  
\end{tabular}}} & 1 & 1.5 \\
\cline{3-4}
%
&& 8 & 1.5 \\
\cline{2-4}
% 
&\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
GPT2-L
\end{tabular}}}  & 1 & 5.1 \\
\cline{3-4}
%
& & 8 & 5.1 \\
\cline{2-4}
% 
&\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
GPT2-XL
\end{tabular}}} & 1 & 11.1 \\
\cline{3-4}
%
& & 8 & 11.3 \\
\cline{2-4}
% 
& \multirow{2}{*}{Llama2} &   1 & 96.1 \\
\cline{3-4}
%
&  & 8 & 96.3 \\
\cline{2-4}
% 
&\multirow{2}{*} {bert} &   1 & 1.4 \\
\cline{3-4}
&  & 8 & 1.4 \\
\hline
%
\end{tabular}
\label{tab:energy}
\vspace{-4mm}
\end{table}
\end{center}

==> Tables/tab_expensive_ops.tex <==
\begin{center}
\begin{table}
\caption{\TODO{Update Task Domain Column}Most time-consuming non-GEMM operator groups for selected Models (Platform A, with GPU acceleration).}

\scriptsize
\centering

\begin{tabular} {   | c | c | c | c | c |  } 
\hline


\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Task \\ Domain
\end{tabular}} 
&
\multirow{2}{*}{
Model}
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Batch  \\ Size  
\end{tabular}} 
& 

\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Operator  \\ Group  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\% of Exec.  \\ Time  
\end{tabular}} 
\\

&&&& \\

% \textbf{ Application } & \textbf{ Models } & \textbf{Batch} & \textbf{ Operator Group } & \textbf{\% of Exec.} 
%
%  &   &  \textbf{Size}& \textbf{Group }   & \textbf{Time }  \\
\hline
%
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Image  \\ Classification
\end{tabular}}
} &\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Vt-b    
\end{tabular}}
}  & 1 &  Norm  & 15 \\ 
\cline{3-5} 
% 
 & & 8 & Norm & 13  \\ 
\hline %\cline{2-5} 
%
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 ViT  \\ Large 16  
\end{tabular}}} 
% 
& \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Vt-l 
\end{tabular}}} & 1 & Norm & 15 \\ 
\cline{3-5}
%
&& 8 & Norm & 12 \\ 
\hline
% 
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Tiny  
\end{tabular}}} & \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Sw-t  
\end{tabular}}}& 1 & Memory & 33.6 \\ 
\cline{3-5}
%
&& 8 & Memory & 30 \\ 
\hline
% 
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Small  
\end{tabular}}} &\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Sw-s  
\end{tabular}}}& 1 & Memory & 34 \\ 
\cline{3-5}
% 
 & & 8 & Memory & 31  \\
\hline
% 
 \multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Base   
\end{tabular}}} &\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
Sw-b   
\end{tabular}}} & 1 & Memory & 34 \\ 
\cline{3-5}
% 
&& 8 & Memory & 31 \\
\hline
%
\multirow{2}{*}{FasterRCNN} &  \multirow{2}{*}{FRCNN}& 1 & Memory & 38 \\ 
\cline{3-5}
%
&& 8 & Memory & 27 \\
\hline
%
 \multirow{2}{*}{MaskRCNN} &  \multirow{2}{*}{MRCNN} & 1 & Memory & 37\\
\cline{3-5}
%
&& 28 & Memory & 49 \\ 
\hline 
% 
 DETR & DETR & 1 & Norm & 34 \\ 
\hline 
%
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 GPT2  \\  
\end{tabular}}} & \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
gpt2  
\end{tabular}}}& 1 & Act & 30 \\
\cline{3-5}
%
& &8 & Act & 30 \\ 
\hline
%
\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
 GPT2  \\ X-Large 
\end{tabular}}}&\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
GPT2-XL
\end{tabular}}} & 1 & Act & 28 \\
\cline{3-5}
%
&& 8 & Act & 28 \\ 
\hline
%
 Llama2-7B & Llama2& 1 &   Norm & 14 \\
\hline
%
\multirow{2}{*} {Bert} &\multirow{2}{*} {bert}& 1 &   Norm & 13 \\
\cline {3-5}
%
&& 8 &   Norm & 13 \\ 
\hline

\end{tabular}
\label{tab:expensive_ops}

\end{table}
\end{center}

==> Tables/tab_expensive_ops_new.tex <==
\begin{table}
\caption{Most time-consuming non-GEMM operator groups for selected Models (Platform A, with GPU acceleration, average across batch sizes).}

\scriptsize
\centering

\begin{tabular} {   | c | c | c | c |  } 
\hline


\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\textbf{Task} \\ \textbf{Domain}
\end{tabular}} 
&
\multirow{2}{*}{
\textbf{Model}}
& 

\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\textbf{Operator}  \\ \textbf{Group}  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\textbf{Latency} \\ \textbf{Percentage (\%)}  
\end{tabular}} 
\\

&&& \\

% \textbf{ Application } & \textbf{ Models } & \textbf{Batch} & \textbf{ Operator Group } & \textbf{\% of Exec.} 
%
%  &   &  \textbf{Size}& \textbf{Group }   & \textbf{Time }  \\
\hline
%
\multirow{6}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Image  \\ Classification
\end{tabular}}
}
% 
&\multirow{1}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Vt-b    
\end{tabular}}
}  
% 
 &  Norm  & 14.0 \\ 
\cline{2-4}
% 
& \multirow{1}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Vt-l 
\end{tabular}}}  & Norm & 13.3 \\ 
\cline{2-4}
%
& \multirow{1}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Vt-h 
\end{tabular}}}  & Norm & 11.2 \\ 
\cline{2-4}
% 
& \multirow{1}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Sw-t  
\end{tabular}}} & Memory & 31.8 \\ 
\cline{2-4}

% 
&\multirow{1}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Sw-s  
\end{tabular}}} & Memory & 33.1 \\ 
\cline{2-4}
% 

&\multirow{1}{*}{{
\begin{tabular}[c]{@{}c@{}} 
Sw-b   
\end{tabular}}}  & Memory & 32.8 \\ 
\hline
% 
\multirow{3}{*}{Object Detection} 
&  \multirow{1}{*}{FRCNN}
& Elmt-wise Arith. & 34.4 \\ 
\cline{2-4}
%
&  \multirow{1}{*}{MRCNN}  & Elmt-wise Arith. & 33.6\\
\cline{2-4}
% 
& DETR & Norm & 34.8 \\ 
\hline
% 
\multirow{2}{*}{Image Segmenation} 
&  \multirow{1}{*}{MF}
& Memory & 40.8 \\ 
\cline{2-4}
%
&  \multirow{1}{*}{Seg}  & Normalization & 17.4\\
\hline
% 
\multirow{5}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 NLP \\  
\end{tabular}}} 
& \multirow{1}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
gpt2  
\end{tabular}}} & Act & 30.2 \\
\cline{2-4}
%
&\multirow{1}{*}{{
\begin{tabular}[c]{@{}c@{}} 
GPT2-L
\end{tabular}}}  & Act & 29.9 \\
\cline{2-4}
%
% 
&\multirow{1}{*}{{
\begin{tabular}[c]{@{}c@{}} 
GPT2-XL
\end{tabular}}} & Act & 28.1 \\
\cline{2-4}
%
& Llama2 &   Norm & 14.9 \\
\cline{2-4}
%
&\multirow{1}{*} {bert} &   Norm & 13.1 \\
\cline{2-4}
&\multirow{1}{*} {Mixtral} &   Memory & 43.1  \\
\hline 
%
\end{tabular}
\label{tab:expensive_ops_new}
\vspace{-0mm}
\end{table}

==> Tables/tab_expensive_ops_old.tex <==
\begin{center}
\begin{table}
\caption{\bench Most Expensive NonGEMM Operator Group for selected \bench Models Running on Data Center GPU Platform.}

\scriptsize
\centering

\begin{tabular} {  |c | c | c | c | c |  } 
\hline

\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Application  \\  
\end{tabular}} 
& 
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Models  \\  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Batch  \\ Size  
\end{tabular}} 
& 
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Operator  \\ Group  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\% of Exec.  \\ Time  
\end{tabular}} 
\\

&&&& \\

% \textbf{ Application } & \textbf{ Models } & \textbf{Batch} & \textbf{ Operator Group } & \textbf{\% of Exec.} 
%
%  &   &  \textbf{Size}& \textbf{Group }   & \textbf{Time }  \\
\hline
%
\multirow{9}{*}{
\begin{tabular}[c]{@{}c@{}} 
Image  \\ Classification 
\end{tabular}} 
& \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 ViT  \\ Base 16  
\end{tabular}}
} & 1 & Norm  & 20 \\ 
\cline{3-5} 
% 
&  & 8 & Norm & 17  \\ 
\cline{2-5} 
%
& \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 ViT  \\ Large 16  
\end{tabular}}} & 1 & Norm & 20.5 \\ 
\cline{3-5}
%
&& 8 & Arith & 17 \\ 
\cline{2-5}
% 
& \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Tiny  
\end{tabular}}} & 1 & Norm & 19 \\ 
\cline{3-5}
%
&& 8 & Norm & 18.5 \\ 
\cline {2-5}
% 
& \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Small  
\end{tabular}}} & 1 & Norm & 18 \\ 
\cline{3-5}
% 
& & 8 & Norm & 17  \\
\cline{2-5}
% 
& \multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Base   
\end{tabular}}} & 1 & Norm & 18 \\ 
\cline{3-5}
% 
&& 8 & Norm & 18 \\
\hline
%
\multirow{7}{*}{Object Detection} & \multirow{3}{*}{FasterRCNN} & 1 & Norm & 60.5 \\ 
\cline{3-5}
%
&& 2 & Norm & 59 \\
\cline {3-5}
%
&& 8 & Norm & 49 \\
\cline {2-5}
%
& \multirow{3}{*}{MaskRCNN} & 1 & Norm & 58\\
\cline{3-5}
%
&& 2 & Norm & 56 \\ 
\cline {3-5}
% 
&& 8 & Norm & 49 \\ 
\cline {2-5}
% 
& DETR & 2 & Norm & 40 \\ 
\hline 
%
\multirow{7}{*}{Language Models} & \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 GPT2  \\  
\end{tabular}}} & 1 & Act & 23 \\
\cline{3-5}
%
&& 64 & Act & 16 \\ 
\cline {2-5}
%
& \multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
 GPT2  \\ X-Large 
\end{tabular}}} & 1 & Act & 23 \\
\cline{3-5}
%
&& 64 & Act & 9 \\ 
\cline {2-5}
%
& Llama2-7B & 1 &   Arith & 23 \\
\cline {2-5}
%
&\multirow{2}{*} {Bert} & 1 &   Arith & 20 \\
\cline {3-5}
%
&& 64 &   Arith & 10 \\ 
\hline

\end{tabular}
\label{tab:expensive_ops}

\end{table}
\end{center}

==> Tables/tab_expensive_ops_shrinked.tex <==
\begin{center}
\begin{table}
\caption{Most Expensive non-GEMM Operator Group for selected Models Running on Data Center GPU Platform. \TODO{Update \% of exec time}}

\scriptsize
\centering

\begin{tabular} {   | c | c | c | c | c |  } 
\hline


\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Models  \\  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Model  \\ Alias  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Batch  \\ Size  
\end{tabular}} 
& 

\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Operator  \\ Group  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\% of Exec.  \\ Time  
\end{tabular}} 
\\

&&&& \\

% \textbf{ Application } & \textbf{ Models } & \textbf{Batch} & \textbf{ Operator Group } & \textbf{\% of Exec.} 
%
%  &   &  \textbf{Size}& \textbf{Group }   & \textbf{Time }  \\
\hline
%
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 ViT  \\ Base 16  
\end{tabular}}
} &\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Vt-b    
\end{tabular}}
}  & 1 &  Norm  & 20 \\ 
\cline{3-5} 
% 
 & & 8 & Norm & 17  \\ 
\hline %\cline{2-5} 
%
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 ViT  \\ Large 16  
\end{tabular}}} & \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Vt-l 
\end{tabular}}} & 1 & Norm & 20.5 \\ 
\cline{3-5}
%
&& 8 & Norm & 17 \\ 
\hline
% 
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Tiny  
\end{tabular}}} & \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Sw-t  
\end{tabular}}}& 1 & Memory & 19 \\ 
\cline{3-5}
%
&& 8 & Memory & 18.5 \\ 
\hline
% 
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Small  
\end{tabular}}} &\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Sw-s  
\end{tabular}}}& 1 & Memory & 18 \\ 
\cline{3-5}
% 
 & & 8 & Memory & 17  \\
\hline
% 
 \multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Base   
\end{tabular}}} &\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
Sw-b   
\end{tabular}}} & 1 & Memory & 18 \\ 
\cline{3-5}
% 
&& 8 & Memory & 18 \\
\hline
%
\multirow{3}{*}{FasterRCNN} &  \multirow{3}{*}{FRCNN}& 1 & Memory & 60.5 \\ 
\cline{3-5}
%
& &2 & Memory & 59 \\
\cline {3-5}
%
&& 8 & Memory & 49 \\
\hline
%
 \multirow{3}{*}{MaskRCNN} &  \multirow{3}{*}{MRCNN} & 1 & Memory & 58\\
\cline{3-5}
%
&& 2 & Memory & 56 \\ 
\cline {3-5}
% 
&& 8 & Memory & 49 \\ 
\hline 
% 
 DETR & DETR & 1 & Norm & 40 \\ 
\hline 
%
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 GPT2  \\  
\end{tabular}}} & \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
gpt2  
\end{tabular}}}& 1 & Act & 23 \\
\cline{3-5}
%
& &8 & Act & 16 \\ 
\hline
%
\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
 GPT2  \\ X-Large 
\end{tabular}}}&\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
GPT2-XL
\end{tabular}}} & 1 & Act & 23 \\
\cline{3-5}
%
&& 8 & Act & 9 \\ 
\hline
%
 Llama2-7B & Llama2& 1 &   Norm & 23 \\
\hline
%
\multirow{2}{*} {Bert} &\multirow{2}{*} {bert}& 1 &   Norm & 20 \\
\cline {3-5}
%
&& 8 &   Norm & 10 \\ 
\hline

\end{tabular}
\label{tab:expensive_ops}

\end{table}
\end{center}

==> Tables/tab_experiment_settings.tex <==
% \begin{center}
% \begin{table}
% \centering
% \scriptsize
% \caption{Hardware platform configurations used for \bench case studies.}
% \begin{tabular} {| l | l | l |}
% \hline
% \multicolumn{1}{|c|}{\textbf{Class}} & \multicolumn{1}{|c|}{\textbf{CPU}} & \multicolumn{1}{|c|}{\textbf{GPU}} \\
% \hline 
% Data Center & AMD EPYC 7763 & NVIDIA A100 \\
% \hline
% Workstation & Intel i9-13900K & NVIDIA RTX 4090 \\
% \hline
% Mobile & Intel i7-13700HU & NVIDIA RTX 4060m \\
% \hline
% \end{tabular}
% \label{tab:experiment_settings}

% \end{table}
% \end{center}





\begin{table}[]
\centering
\scriptsize
\caption{Hardware platform configurations used for case studies.}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{ID}}} 
& \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Class}}} 
& \multicolumn{1}{c|}{\multirow{1}{*} {\textbf{CPU}}}             
& \multicolumn{3}{c|}{\multirow{1}{*}{\textbf{GPU}}}
\\ 
\cline{3-6}
%%
&
& \multicolumn{1}{c|}{\textbf{Device}}             
& \multicolumn{1}{c|}{\textbf{Device}}             
& \multicolumn{1}{c|}{\textbf{Mem.}}
& \multicolumn{1}{c|}{\textbf{TOPS}} \\ 
\hline
%%
A
& Data Center                                   
& \multicolumn{1}{l|}{AMD EPYC 7763}                           
& \multicolumn{1}{l|}{Nvidia A100}      
& \multicolumn{1}{r|} {80 GB}
& \multicolumn{1}{r|} {624} \\ 
\hline
%%
B
& Workstation                                  
& \multicolumn{1}{l|}{Intel i9-13900K}                         
& \multicolumn{1}{l|}{Nvidia RTX 4090}  
& \multicolumn{1}{r|} {24 GB}
& \multicolumn{1}{r|} {660} \\ 
\hline
%%
\end{tabular}
\vspace{-5mm}
\label{tab:experiment_settings}
\end{table}

==> Tables/tab_fusion_rate.tex <==
\begin{table}[t]
\caption {The non-GEMM latency before and after applying fusion with TensorRT. The values between brackets represent the percentage with resect to the total inference latency.}

\centering

\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Model}}} 
% 
& \multicolumn{1}{c|}{\multirow{1}{*}{\textbf{Non-GEMM}}} 
% 
& \multicolumn{2}{c|}{\multirow{1}{*}{\textbf{Non-GEMM Latency}}} \\ 
\cline{3-4}
& \multirow{1}{*}{\textbf{Fusion Rate}}
& \multirow{1}{*}{\textbf{Before Fusion}} 
& \multirow{1}{*}{\textbf{After Fusion}} \\
\hline
% 

\multicolumn{1}{|c|}{Swin-t}  
& \multicolumn{1}{r|}{8.8\%}
% 
& \multicolumn{1}{r|}{7.53 ms (\textit{56.4\%})}
& \multicolumn{1}{r|}{0.97 ms (\textit{39.0\%})} \\ 
\hline
% 
\multicolumn{1}{|c|}{Swin-b}  
& \multicolumn{1}{r|}{7.0\%}
& \multicolumn{1}{r|}{14.59 ms (\textit{56.4\%})}
& \multicolumn{1}{r|}{1.65 ms (\textit{32.3\%})} \\ 
\hline
% 
\multicolumn{1}{|c|}{DETR}  
& \multicolumn{1}{r|}{30.0\%}
& \multicolumn{1}{r|}{32.17 ms (\textit{66.4\%})}
& \multicolumn{1}{r|}{2.38 ms (\textit{18.5\%})} \\ 
\hline
% 
\multicolumn{1}{|c|}{Segformer}  
& \multicolumn{1}{r|}{27.0\%}
& \multicolumn{1}{r|}{5.57 ms (\textit{41.0\%})}
& \multicolumn{1}{r|}{2.33 ms (\textit{41.0\%})} \\ 
\hline
% 
\end{tabular}
\label{tab:fusion_rate}
\vspace{-2mm}
\end{table}


% \begin{table}[]
% \caption {Fusion Rate \TODO{ADD before Fusion and After Fusion, show raw latency ideally}}

% \centering

% \begin{tabular}{|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{Model} 
% % 
% & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Non-GEMM \\ Fusion Rate\end{tabular}} 
% % 
% & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Non-GEMM\\Latency Pct\end{tabular}} \\ 
% \hline
% Swin-b 
% % 
% & \multicolumn{1}{r|}{7\%}
% % 
% & \multicolumn{1}{r|}{32.25\%} \\ 
% \hline

% DETR 
% & \multicolumn{1}{r|} {30\%} 
% & \multicolumn{1}{r|}{18.5\%} \\
% \hline
% Segformer
% % 
% & \multicolumn{1}{r|}{27\%} 
% & \multicolumn{1}{r|}{41\%}\\ 
% \hline
% Llama 2
% & \multicolumn{1}{r|}{27\%} 
% &  \multicolumn{1}{r|}{17.5\%} \\ \hline
% \end{tabular}
% \label{tab:fusion_rate}
% \end{table}

==> Tables/tab_hw.tex <==
% --- Table for Hardware Specifications ---
% \begin{table*}[t]
\begin{table}[t]
\centering
\caption{Evaluation Setup for Consumer and Embedded GPU Platforms.}
\label{tab:gpu_setup}
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Specification} & \textbf{GPU 1 (Consumer)} & \textbf{GPU 2 (Edge)} \\ \midrule
GPU Model                        & NVIDIA RTX 4090           & NVIDIA Jetson Orin Nano$^1$   \\
Architecture                     & Ada Lovelace              & Ampere                    \\
% Streaming Multiprocessors (SMs)  & 128                       & 8                         \\
SMs  & 128                       & 8                         \\
% Computation Throughput (FP16/BF16)$^1$           & $\sim$330 TFLOPS          & $\sim$20 TFLOPS           \\
Comp. Throughput           & $\sim$330 TFLOPS          & $\sim$20 TFLOPS           \\
GPU Memory                       & 24 GB GDDR6X              & 8 GB LPDDR5 (Shared)      \\
Memory Bandwidth                 & 1008 GB/s                 & 68 GB/s                   \\
Host Interconnect                & PCIe 4.0, 16x             & Integrated on-chip        \\ \bottomrule
% \multicolumn{3}{l}{\footnotesize $^1$ Approximate TFLOPS for dense operations.}
% \multicolumn{3}{l}{\footnotesize $^1$ (FP16/BF16) Approximate TFLOPS for dense operations.}
\multicolumn{3}{l}{\footnotesize $^1$ \texttt{MAXN} power mode enabled with 16GB swap from NVMe}
\end{tabular}
% \end{table*}
\end{table}

==> Tables/tab_hybrid_ssm_compare.tex <==
% --- First Part of the Table ---
\begin{table*}[htbp] % Use table* for spanning two columns
  \caption{Comparison of Recent Hybrid Transformer-SSM Language Models (Part 1 of 2)} % Modified caption
  \label{tab:hybrid_model_comparison} % Original label is here
  \scriptsize % Adjust font size if needed

\begin{tabularx}{\linewidth}{XXXXXXXXXX} % Use \linewidth for tabularx within table*
    \toprule
    \textbf{Name} & \textbf{Date Released/ Venue} & \textbf{Supplier} & \textbf{Paper Link} & \textbf{Open Weights} & \textbf{Framework req} & \textbf{Special SW} & \textbf{Special HW} & \textbf{Pro Result / Feature Diff} & \textbf{Con Result / Limitation } \\
    \midrule

    \textbf{Jamba} & Mar 2024 & AI21 Labs & \href{https://arxiv.org/abs/2403.19887}{arXiv:2403.19887} & Yes (Apache 2.0) & PyTorch, HF Transformers & `mamba-ssm`, `causal-conv1d` & 80GB GPU (Target) & MoE for scaling capacity; Very low KV cache (4GB @ 256K); High throughput on long context (3x Mixtral); 256K context support. & MoE complexity (training, deployment); Size is huge Jamba Mini 1.6 (12B active/52B total) and Jamba Large 1.6 (94B active/398B total), needs 2 80GB A100 GPUs and default vLLM configuration for 200k tokens. \\
    \addlinespace % Add a bit of vertical space

    \textbf{SAMBA} & Jun 2024; ICLR 2025 & Microsoft & \href{https://arxiv.org/abs/2406.07522}{arXiv:2406.07522} & Code Sample Only & PyTorch & `mamba-ssm`, Custom SWA? & Standard GPUs & Unlimited context extrapolation (tested to 1M); Linear time complexity; High throughput (3.6x-3.7x vs Llama-3 GQA); Perfect passkey recall (256K) after tuning. & Simple interleaving architecture; Numbers are good but base weights not released. \\
    \addlinespace

    \textbf{8B Mamba2-Attention Hybrid} & June 2024 & NVIDIA; CMU; Princeton; Together AI & \href{https://arxiv.org/abs/2406.07887}{arXiv:2406.07887} & ? & \href{https://github.com/NVIDIA/Megatron-LM/tree/main/examples/mamba}{Megatron-LM} & `mamba-ssm`, `causal-conv1d` &   & Initial study collaborating with Mamba authors before NVIDIA picked up hybrid SSM. Demonstrated that a hybrid architecture incorporating only a small fraction of self-attention layers strategically interspersed within the Mamba-2 backbone exceeded the performance of the pure Transformer baseline on average across 12 standard tasks (+2.65 points) & Emperical study \\

    \bottomrule
  \end{tabularx}
\end{table*}
% --- End of First Part ---

% --- Add \clearpage if you want to force the next table onto a new page ---
% \clearpage 
% --- Or let LaTeX place it naturally, likely at the top of the next page ---

% --- Second Part of the Table ---
\begin{table*}[htbp] % Start the second table spanning two columns
  \caption*{Table \ref{tab:hybrid_model_comparison} Continued: Comparison of Recent Hybrid Transformer-SSM Language Models (Part 2 of 2)} % Use \caption* for continuation
  \scriptsize % Keep font size consistent

\begin{tabularx}{\linewidth}{XXXXXXXXXX} % Use \linewidth, same column specifiers
    \toprule
    % --- Repeat the headers ---
    \textbf{Name} & \textbf{Date Released} & \textbf{Supplier} & \textbf{Paper Link} & \textbf{Open Weights} & \textbf{Framework req} & \textbf{Special SW} & \textbf{Special HW} & \textbf{Pro Result / Feature Diff} & \textbf{Con Result / Limitation } \\
    \midrule
    % --- Continued data rows ---
    \textbf{Zamba2} & Nov 2024 & Zyphra & \href{https://arxiv.org/abs/2411.15242}{arXiv:2411.15242} & Yes (Apache 2.0, +Dataset) & PyTorch, HF Transformers & `mamba-ssm` & Standard GPUs & SOTA for size class (1.2B-7.4B); Highly efficient inference (Faster TTFT, 6x less KV cache); Parameter-efficient shared attention + LoRA design. & \\
    \addlinespace

    \textbf{Hymba} & Nov 2024; ICLR 2025 & NVIDIA & \href{https://arxiv.org/abs/2411.13676}{arXiv:2411.13676} & Yes (Base, Instruct) & PyTorch, NVIDIA Frameworks? & `mamba-ssm`, Custom kernels? & Standard NVIDIA GPUs & Novel parallel hybrid-headLlama-3-8B; Meta tokens; Very cache efficient (11.7x < Llama-3.2-1B); High throughput (3.5x > Llama-3.2-1B); SOTA for small LMs (<2B). & Paper focuses on small models; Parallel head fusion complexity. Only supports CUDA 12.1/12.4, need to configure pinnacles to run this, however a docker container is available, yet to try\\
    \addlinespace

    \textbf{Nemotron-H} & Apr 16, 2025 & NVIDIA & \href{https://arxiv.org/abs/2504.03624}{arXiv:2504.03624} & Yes (Base) & PyTorch, NeMo 24.12, HF Transformers & `mamba-ssm`, Transformer Engine (FP8), MiniPuzzle (internal) & H100-80GB (for FP8), A100 & High accuracy; Very high inference speed (up to 3x > Transformers); FP8 training capability; MiniPuzzle compression enables smaller deployments (e.g., 47B on 32GB GPU). & FP8 requires specific HW/SW; Relies on NVIDIA ecosystem \\

    \bottomrule
  \end{tabularx}
\end{table*}
% --- End of Second Part ---


% \begin{table*}[htbp] % Use table* for spanning two columns
%   \caption{Comparison of Recent Hybrid Transformer-SSM Language Models}
%   \label{tab:hybrid_model_comparison}
%   \scriptsize % Adjust font size if needed (e.g., \footnotesize, \scriptsize)

%   % \begin{tabularx}{\textwidth}{@{} l l l l l l l l l l @{}} % Use tabularx, define column types. L allows wrapping.
% \begin{tabularx}{\linewidth}{XXXXXXXXXX}
%     \toprule
%     \textbf{Name} & \textbf{Date Released} & \textbf{Supplier} & \textbf{Paper Link} & \textbf{Open Weights} & \textbf{Framework req} & \textbf{Special SW} & \textbf{Special HW} & \textbf{Pro Result / Feature Diff} & \textbf{Con Result / Limitation } \\
%     \midrule


    

    
%     \textbf{Jamba} & Mar 2024 & AI21 Labs & \href{https://arxiv.org/abs/2403.19887}{arXiv:2403.19887} & Yes (Apache 2.0) & PyTorch, HF Transformers & `mamba-ssm`, `causal-conv1d` & 80GB GPU (Target) & MoE for scaling capacity; Very low KV cache (4GB @ 256K); High throughput on long context (3x Mixtral); 256K context support. & MoE complexity (training, deployment); Size is huge  Jamba Mini 1.6 (12B active/52B total) and Jamba Large 1.6 (94B active/398B total), needs 2 80GB A100 GPUs and default vLLM configuration for 200k tokens. \\
%     \addlinespace % Add a bit of vertical space

%     \textbf{SAMBA} & Jun 2024 & Microsoft & \href{https://arxiv.org/abs/2406.07522}{arXiv:2406.07522} & Code Sample Only & PyTorch & `mamba-ssm`, Custom SWA? & Standard GPUs & Unlimited context extrapolation (tested to 1M); Linear time complexity; High throughput (3.6x-3.7x vs Llama-3 GQA); Perfect passkey recall (256K) after tuning. & Simple interleaving architecture; Numbers are good but base weights not released. \\
%     \addlinespace

%     \textbf{8B Mamba2-Attention Hybrid} & June 2024 & NVIDIA; CMU; Princeton; Together AI & \href{https://arxiv.org/abs/2406.07887}{arXiv:2406.07887} & ? & \href{https://github.com/NVIDIA/Megatron-LM/tree/main/examples/mamba}{Megatron-LM} & `mamba-ssm`, `causal-conv1d` &  & Initial study collaborating with Mamba authors before NVIDIA picked up hybrid SSM. Demonstrated that a hybrid architecture incorporating only a small fraction of self-attention layers strategically interspersed within the Mamba-2 backbone exceeded the performance of the pure Transformer baseline
% on average across 12 standard tasks (+2.65 points & Emperical study \\
%     \addlinespace % Add a bit of vertical space

%     \textbf{Zamba2} & Nov 2024 & Zyphra & \href{https://arxiv.org/abs/2411.15242}{arXiv:2411.15242} & Yes (Apache 2.0, +Dataset) & PyTorch, HF Transformers & `mamba-ssm` & Standard GPUs & SOTA for size class (1.2B-7.4B); Highly efficient inference (Faster TTFT, 6x less KV cache); Parameter-efficient shared attention + LoRA design. & \\
%     \addlinespace

%     \textbf{Hymba} & Nov 2024 & NVIDIA & \href{https://arxiv.org/abs/2411.13676}{arXiv:2411.13676} & Yes (Base, Instruct) & PyTorch, NVIDIA Frameworks? & `mamba-ssm`, Custom kernels? & Standard NVIDIA GPUs & Novel parallel hybrid-head; Meta tokens; Very cache efficient (11.7x < Llama-3.2-1B); High throughput (3.5x > Llama-3.2-1B); SOTA for small LMs (<2B). & Paper focuses on small models; Parallel head fusion complexity. Only supports CUDA 12.1/12.4, need to configure pinnacles to run this, however a docker container is available, yet to try\\
%     \addlinespace

%     \textbf{Nemotron-H} & Apr 16, 2025 & NVIDIA & \href{https://arxiv.org/abs/2504.03624}{arXiv:2504.03624} & Yes (Base) & PyTorch, NeMo 24.12, HF Transformers & `mamba-ssm`, Transformer Engine (FP8), MiniPuzzle (internal) & H100-80GB (for FP8), A100 & High accuracy; Very high inference speed (up to 3x > Transformers); FP8 training capability; MiniPuzzle compression enables smaller deployments (e.g., 47B on 32GB GPU). & FP8 requires specific HW/SW; Relies on NVIDIA ecosystem \\

%     \bottomrule
%   \end{tabularx}
% \end{table*}

% % \balance % Optional: Balances columns on the last page


==> Tables/tab_microbench.tex <==
\begin{center}
\begin{table*}
\centering
\caption{A list of non-GEMM operators collected from eight popular model variants selected from Hugging Face listed in~\autoref{tab:modeltable}.\HK{I suggest to add one more column that shows the number of different input shapes/arguments in NonGEMM Bench} \RK{Add the characteristics of each operator}}
\scriptsize

\begin{tabular} {| c | c |  c | c | c |c| c | c| c|}
\hline 

\textbf{Operator Group}
% \multicolumn{1}{|c|}{\textbf{Operator Group}} 



& \multicolumn{1}{c|}{
\textbf{Operator}} 


& \multicolumn{1}{c|}{\textbf{Model}}


& \multicolumn{1}{c|}{\textbf{Single Operation}}


& \multicolumn{1}{c|}{\textbf{Single Operand}}


& \multicolumn{1}{c|}{\textbf{Non-Linearity}}


& \multicolumn{1}{c|}{\textbf{Dynamicity}}


& \multicolumn{1}{c|}{\textbf{Reduction}}



& \multicolumn{1}{c|}{\textbf{\# Input Shapes}} \\

\hline 

\multirow{4}{*}{Activation}
& ReLu 
& DETR
& \checkmark
& \checkmark
&  %checkmark
&  %\checkmark
&  %\checkmark
%Torch.nn.modules.activation
& \checkmark \\%\tiny [2,64,533],  \\
\cline{2-9} 

& GELU
& ViT-l16
%Torch.nn.modules.activation
& \checkmark
& \checkmark
& \checkmark
& 
& 
& \checkmark \\%\tiny [1, 97, 4096] \\
\cline{2-9}

& GELU 
& GPT2-XL 
%transformers.activations.GELUActivation
& \checkmark
& \checkmark
& \checkmark
&  
&  
& \checkmark \\%\tiny [1, 8, 6400] \\
\cline{2-9}

& SiLu 
& Llama-2 
& \checkmark %Torch.nn 
& \checkmark
& \checkmark
&  
& 
& \checkmark \\  %\tiny [1, 10, 11008]\\%, [1, 66, 11008], [1,338,11008] \\
\hline 


\multirow{6}{*}{Normalization}
& LayerNorm
& Segformer
&  %Torch.nn.modules.normalization
& \checkmark
& \checkmark
&  
& \checkmark
& \checkmark \\%\tiny [2, 16384, 32]\\%, [2, 256, 32], [2, 4096, 64] \\
\cline{2-9} 

& BatchNorm2d
& Segformer
&   %Torch.nn.modules.batchnorm
& \checkmark
& \checkmark
&  
& \checkmark
& \checkmark \\%\tiny [2, 256, 128, 128]\\% \\
\cline{2-9} 

& LlamaRMSNorm
& Llama
&  %transformers.models.llama
& \checkmark
& \checkmark
&  
& \checkmark
& \checkmark \\%\tiny [1, 10, 4096]\\%, [1,338,4096], [1,118,4096]    \\ 
\cline{2-9} 

& FrozenBatchNorm2d
& MaskRCNN
&   %torchvision.ops.misc
& \checkmark
& \checkmark
&  
& \checkmark
& \checkmark \\%\tiny [1, 1024, 50,68]\\%, [1, 256, 100, 136] \\
\cline{2-9} 

& FrozenBatchNorm2d
& DETR
&   %transformers.models.detr
& \checkmark
& \checkmark
&  
& \checkmark
& \checkmark \\%\tiny [2, 850, 256] \\
\cline{2-9} 

& LayerNorm
& DETR
&   %Torch.nn.modules.normalization
& \checkmark
& \checkmark
&  
& \checkmark

& \checkmark \\%\tiny [2, 850, 256]\\%, [2, 100, 256] \\
\hline 

\multirow{5}{*}{ Arithmetic} 
& Add
& Segformer
& \checkmark %Torch.add
&  
&  
&  
& 
& \checkmark \\%\tiny [2, 16384, 32]\\%, [2, 4096, 64], [2, 256, 256] \\
\cline{2-9} 

& Mul
& Llama-2
& \checkmark  %Torch.mul
&  
&  
&  
&  
& \checkmark \\%\tiny [1, 10, 11008]\\%, [1, 66, 11008] \\ 
\cline{2-9} 

& Neg
& Llama-2
& \checkmark %Torch.neg
&  
&  
&  
&  
& \checkmark \\%\tiny [1, 32, 10, 64] \\
\cline{2-9} 


& TrueDiv
& Segformer 

& \checkmark %Torch.true\_divide
&  
&  
&  
&  
& \checkmark \\%\tiny [2, 1, 16384, 256]\\%, [2, 8, 256, 256] \\
\cline{2-9} 

& TrueDiv 
& GPT2-XL
& \checkmark %Torch.true\_divide
&  
&  
&  
&  
& \checkmark \\%\tiny [1, 25, 8, 8] \\
\hline 

% contiguous & Memory Op & Returns a new allocated tensor in a specified memory format \cite{paszke2019pytorch} & [391, 144, 4, 32] \\ 
% \hline 

% permute & Memory Op &  Returns a different view of the tensor based on the specified dimensions ~\cite{paszke2019pytorch} & [782, 144, 4, 32] \\ 
% \hline 

% view & Memory Op  & Allocates a new tensor in memory with same data as the input but with different shapes & [391, 12, 12, 1] \\ 
% \hline 


\multirow{9}{*}{Memory}  
& Contiguous
& Segformer
& \checkmark %Torch.Tensor.contiguous
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [2, 32, 128, 128]\\%, [2, 4096, 2, 32], [2, 64, 64, 64] \\
\cline{2-9} 

& Contiguous
& Llama-2
& \checkmark %Torch.Tensor
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [1, 10, 32, 128]\\%, [1, 118, 32, 128] \\
\cline{2-9} 

& Permute
& ViT-b16
& \checkmark %Torch.permute
& \checkmark
&  
& 
&  
& \checkmark \\%\tiny [1, 768, 196]\\% \\ 
\cline{2-9} 

& Permute
& GPT2-XL
& \checkmark %Torch.permute
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [1, 8, 25, 64] \\
\cline{2-9} 

& Split
& GPT2-XL
& \checkmark %Torch.split
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [1, 8, 4800] \\ 
\cline{2-9} 

& View 
& GPT2-XL
& \checkmark %Torch.Tensor.view
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [1, 8, 1600]\\
\cline{2-9} 

& Reshape
& ViT-b16
& \checkmark %Torch.reshape
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [1, 768, 14, 14]\\
\cline{2-9} 

& Expand
& ViT-b16
& \checkmark %Torch.Tensor.expand
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [1, 1, 768] \\
\cline{2-9} 

& Squeeze
& Llama-2
& \checkmark %Torch.squeeze
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [1, 1, 10, 128] \\ 
\hline 

%\multirow{2}{*}{Logit Computation} 
Logit 
& Softmax 
& DETR 
& \checkmark %Torch.nn.Functional.softmax
& \checkmark
& \checkmark
&  
& \checkmark
& \checkmark \\%\tiny [1, 25, 8, 8] \\ 
\cline{2-9} 

Computation
& Softmax
& Segformer
& \checkmark %Torch.nn.Functional.softmax
& \checkmark
& \checkmark
& 
& \checkmark
& \checkmark \\%\tiny [2, 1, 16384, 256]\\%, [2, 5, 1024, 256] \\ 
\hline 

RoI Selection
& NMS
& MaskRCNN
&  %torchvision.ops.nms
& 
& 
& \checkmark
& 
& \checkmark \\%\tiny [4663, 4] \\ 
\hline 

Interpolation
& Interpolate
& Segformer
&  %
& \checkmark
& 
& 
& 
& \checkmark \\%Torch.nn.Functional
%, [2, 256, 16, 16] \\
\hline 



\end {tabular}
\label{tab:microbench}
\end{table*}
\end{center}

==> Tables/tab_microbench_new.tex <==
\begin{table*}
\centering
\caption{Non-GEMM operators in eight selected model variants from~\autoref{tab:modeltable} and their characteristics. Example input shapes are captured based on inferences using real datasets.}
\scriptsize

\begin{tabular} {| c | c |  c | c | c |c| c | c| c|}
\hline 

\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\textbf{Operator} \\ \textbf{Group}
\end{tabular}}

% \multicolumn{1}{|c|}{\textbf{Operator Group}} 


& \multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\textbf{Operator}
\end{tabular}}

% & \multicolumn{1}{c|}{
% \textbf{Operator}} 


& \multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\textbf{Model}
\end{tabular}}

% & \multicolumn{1}{c|}{\textbf{Model}}

& \multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\textbf{Single} \\ \textbf{Operation}
\end{tabular}}

% & \multicolumn{1}{c|}{\textbf{Single Operation}}

& \multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\textbf{Single} \\ \textbf{Operand}
\end{tabular}}

% & \multicolumn{1}{c|}{\textbf{Single Operand}}

& \multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\textbf{Non} \\ \textbf{Linearity}
\end{tabular}}
% & \multicolumn{1}{c|}{\textbf{Non-Linearity}}

& \multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\textbf{Dynamicity}
\end{tabular}}
% & \multicolumn{1}{c|}{\textbf{Dynamicity}}


& \multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\textbf{Reduction}
\end{tabular}}
% & \multicolumn{1}{c|}{\textbf{Reduction}}


& \multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\textbf{Example} \\ \textbf{Input Shape}
\end{tabular}}
\\
&&&&&&&& \\
% & \multicolumn{1}{c|}{\textbf{\# Input Shapes}} \\

\hline 

\multirow{4}{*}{Activation}
& ReLu 
& DETR
& \checkmark
& \checkmark
&  %checkmark
&  %\checkmark
&  %\checkmark
%Torch.nn.modules.activation
& [2,64,533]\\%\tiny [2,64,533],  \\
\cline{2-9} 

& GELU
& ViT-l16
%Torch.nn.modules.activation
& 
& \checkmark
& \checkmark
& 
& 
& [1, 97, 4096] \\%\tiny [1, 97, 4096] \\
\cline{2-9}

& GELU 
& GPT2-XL 
%transformers.activations.GELUActivation
& 
& \checkmark
& \checkmark
&  
&  
& [1, 8, 6400] \\%\tiny [1, 8, 6400] \\
\cline{2-9}

& SiLu 
& Llama-2 
& 
& \checkmark
& \checkmark
&  
& 
& [1, 10, 11008] \\  %\tiny [1, 10, 11008]\\%, [1, 66, 11008], [1,338,11008] \\
\hline 


\multirow{6}{*}{Normalization}
& LayerNorm
& Segformer
&  %Torch.nn.modules.normalization
& \checkmark
& \checkmark
&  
& \checkmark
& [2, 16384, 32] \\%\tiny [2, 16384, 32]\\%, [2, 256, 32], [2, 4096, 64] \\
\cline{2-9} 

& BatchNorm2d
& Segformer
&   %Torch.nn.modules.batchnorm
& \checkmark
& \checkmark
&  
& \checkmark
& [2, 256, 128, 128] \\%\tiny [2, 256, 128, 128]\\% \\
\cline{2-9} 

& LlamaRMSNorm
& Llama
&  %transformers.models.llama
& \checkmark
& \checkmark
&  
& \checkmark
& [1, 10, 4096] \\%\tiny [1, 10, 4096]\\%, [1,338,4096], [1,118,4096]    \\ 
\cline{2-9} 

& FrozenBatchNorm2d
& MaskRCNN
&   %torchvision.ops.misc
& \checkmark
& \checkmark
&  
& \checkmark
& [1, 1024, 50,68] \\%\tiny [1, 1024, 50,68]\\%, [1, 256, 100, 136] \\
\cline{2-9} 

& FrozenBatchNorm2d
& DETR
&   %transformers.models.detr
& \checkmark
& \checkmark
&  
& \checkmark
& [1, 2048, 25, 34] \\%\tiny [2, 850, 256] \\
\cline{2-9} 

& LayerNorm
& DETR
&   %Torch.nn.modules.normalization
& \checkmark
& \checkmark
&  
& \checkmark

& [2, 850, 256] \\%\tiny [2, 850, 256]\\%, [2, 100, 256] \\
\hline 

\multirow{5}{*}{ Elmt-wise Arithmetic} 
& Add
& Segformer
& \checkmark %Torch.add
&  
&  
&  
& 
& [2, 16384, 32] \\%\tiny [2, 16384, 32]\\%, [2, 4096, 64], [2, 256, 256] \\
\cline{2-9} 

& Mul
& Llama-2
& \checkmark  %Torch.mul
&  
&  
&  
&  
& [1, 10, 11008] \\%\tiny [1, 10, 11008]\\%, [1, 66, 11008] \\ 
\cline{2-9} 

& Neg
& Llama-2
& \checkmark %Torch.neg
&  
&  
&  
&  
& [1, 32, 10, 64] \\%\tiny [1, 32, 10, 64] \\
\cline{2-9} 


& TrueDiv
& Segformer 

& \checkmark %Torch.true\_divide
&  
&  
&  
&  
& [2, 1, 16384, 256] \\%\tiny [2, 1, 16384, 256]\\%, [2, 8, 256, 256] \\
\cline{2-9} 

& TrueDiv 
& GPT2-XL
& \checkmark %Torch.true\_divide
&  
&  
&  
&  
& [1, 25, 8, 8] \\%\tiny [1, 25, 8, 8] \\
\hline 

% contiguous & Memory Op & Returns a new allocated tensor in a specified memory format \cite{paszke2019pytorch} & [391, 144, 4, 32] \\ 
% \hline 

% permute & Memory Op &  Returns a different view of the tensor based on the specified dimensions ~\cite{paszke2019pytorch} & [782, 144, 4, 32] \\ 
% \hline 

% view & Memory Op  & Allocates a new tensor in memory with same data as the input but with different shapes & [391, 12, 12, 1] \\ 
% \hline 


\multirow{9}{*}{Memory}  
& Contiguous
& Segformer
& \checkmark %Torch.Tensor.contiguous
& \checkmark
&  
&  
&  
& [2, 32, 128, 128] \\%\tiny [2, 32, 128, 128]\\%, [2, 4096, 2, 32], [2, 64, 64, 64] \\
\cline{2-9} 

& Contiguous
& Llama-2
& \checkmark %Torch.Tensor
& \checkmark
&  
&  
&  
& [1, 10, 32, 128] \\%\tiny [1, 10, 32, 128]\\%, [1, 118, 32, 128] \\
\cline{2-9} 

& Permute
& ViT-b16
& \checkmark %Torch.permute
& \checkmark
&  
& 
&  
& [1, 768, 196] \\%\tiny [1, 768, 196]\\% \\ 
\cline{2-9} 

& Permute
& GPT2-XL
& \checkmark %Torch.permute
& \checkmark
&  
&  
&  
& [1, 8, 25, 64] \\%\tiny [1, 8, 25, 64] \\
\cline{2-9} 

& Split
& GPT2-XL
& \checkmark %Torch.split
& \checkmark
&  
&  
&  
& [1, 8, 4800] \\%\tiny [1, 8, 4800] \\ 
\cline{2-9} 

& View 
& GPT2-XL
& \checkmark %Torch.Tensor.view
& \checkmark
&  
&  
&  
& [1, 8, 1600] \\%\tiny [1, 8, 1600]\\
\cline{2-9} 

& Reshape
& ViT-b16
& \checkmark %Torch.reshape
& \checkmark
&  
&  
&  
&[1, 768, 14, 14] \\%\tiny [1, 768, 14, 14]\\
\cline{2-9} 

& Expand
& ViT-b16
& \checkmark %Torch.Tensor.expand
& \checkmark
&  
&  
&  
& [1, 1, 768] \\%\tiny [1, 1, 768] \\
\cline{2-9} 

& Squeeze
& Llama-2
& \checkmark %Torch.squeeze
& \checkmark
&  
&  
&  
& [1, 1, 10, 128] \\%\tiny [1, 1, 10, 128] \\ 
\hline 

%\multirow{2}{*}{Logit Computation} 
Logit 
& Softmax 
& DETR 
& \checkmark %Torch.nn.Functional.softmax
& \checkmark
& \checkmark
&  
& \checkmark
& [1, 25, 8, 8] \\%\tiny [1, 25, 8, 8] \\ 
\cline{2-9} 

Computation
& Softmax
& Segformer
& \checkmark %Torch.nn.Functional.softmax
& \checkmark
& \checkmark
& 
& \checkmark
& [2, 1, 16384, 256] \\%\tiny [2, 1, 16384, 256]\\%, [2, 5, 1024, 256] \\ 
\hline 

RoI Selection
& NMS
& MaskRCNN
&  %torchvision.ops.nms
& 
& 
& \checkmark
& 
& [4663, 4] \\%\tiny [4663, 4] \\ 
\hline 

Interpolation
& Interpolate
& Segformer
&  %
& \checkmark
& 
& 
& 
& [2, 256, 128, 128] \\%Torch.nn.Functional
%, [2, 256, 16, 16] \\
\hline 

\end {tabular}
\vspace{-4mm}
\label{tab:microbench}
\end{table*}

==> Tables/tab_microbench_old.tex <==
\begin{center}
\begin{table}
\tiny
\begin{tabular} {| c | c |  c | c | c|}
\hline 
\textbf{Operator} & \textbf{Operator Group} & \textbf{Model} & \textbf{Implementation} & \textbf{Example Input Size} \\
\hline 

GELU & Activation & ViT-l16 & Torch.nn.modules.activation & [1, 97, 4096] \\
\hline

% GELU & Activation & Applies a custom implementation of gelu non linear activation function & [1, 8, 6400] \\
% \hline

% Softmax & Softmax & Applies a function to map the features/logits to probabilities & [1, 25, 8, 8] \\ 
% \hline 

% Tensor Addition & Arithmetic  & Performs an element wise addition on tensors & [[1, 12, 8, 8], [1, 1, 1, 8]] \\
% \hline

% TrueDiv & Arithmetic  & Performs an element wise division on tensors with rounding & [1, 32, 10, 10] \\ 
% \hline 

LlamaRMSNorm & Normalization & Llama & transformers.models.llama &  [1, 10, 4096], [1, 66, 4096], [1,338,4096], [1,118,4096]    \\ 
\hline 



FrozenBatchNorm2d & Normalization & MaskRCNN & torchvision.ops.misc  & [1, 1024, 50,68], [1, 512, 100, 136], [1, 256, 100, 136] \\
\hline 

Filter\_proposals & NMS & MaskRCNN & trochvisino.models.detection.rpn & [4663, 4] \\ 
\hline 

FrozenBatchNorm2d & Normalization & DETR & transformers.models.detr & [2, 850, 256] \\
\hline

% contiguous & Memory Op & Returns a new allocated tensor in a specified memory format \cite{paszke2019pytorch} & [391, 144, 4, 32] \\ 
% \hline 

% permute & Memory Op &  Returns a different view of the tensor based on the specified dimensions ~\cite{paszke2019pytorch} & [782, 144, 4, 32] \\ 
% \hline 

% view & Memory Op  & Allocates a new tensor in memory with same data as the input but with different shapes & [391, 12, 12, 1] \\ 
% \hline 

ReLu & Activation & DETR & Torch.nn.modules.activation &  [2,64,533],  \\
\hline 

LayerNorm & Normalization & DETR  & Torch.nn.modules.normalization & [2, 850, 256], [2, 100, 256] \\
\hline 

Softmax & Softmax & DETR & Torch.nn.Functional & [1, 25, 8, 8] \\ 
\hline 

LayerNorm & Normalization & Segformer  & Torch.nn.modules.normalization & [2, 16384, 32], [2, 256, 32], [2, 4096, 64], [2, 256, 64] \\
\hline 

BatchNorm2d & Normalization & Segformer & Torch.nn.modules.batchnorm & [2, 256, 128, 128] \\
\hline

contiguous & Memory Op & Segformer & Torch.Tensor & [2, 32, 128, 128], [2, 4096, 2, 32], [2, 64, 64, 64] \\
\hline 

Interpolate & Arithmetic & Segformer & Torch.nn.Functional & [2, 256, 128, 128], [2, 256, 64, 64], [2, 256, 32, 32], [2, 256, 16, 16] \\
\hline 

TrueDiv & Arithmetic & Segformer & Torch &  [2, 1, 16384, 256], [2, 2, 4096, 256], [2, 5, 1024, 256], [2, 8, 256, 256] \\
\hline 

Add & Arithmetic & Segformer & Torch & [2, 16384, 32], [2, 4096, 64], [2, 1024, 160], [2, 256, 256] \\
\hline 

Softmax & Softmax & Segformer & Torch.nn.Functional &  [2, 1, 16384, 256], [2, 2, 4096, 256], [2, 5, 1024, 256], [2, 8, 256, 256] \\ 
\hline 

SiLu & Activation & Llama-2 & Torch.nn &  [1, 10, 11008], [1, 66, 11008], [1,338,11008], [1,118,11008]\\
\hline 

mul & Arithmetic & Llama-2 & Torch &[1, 10, 11008], [1, 66, 11008] \\ 
\hline 

neg & Arithmetic & Llama-2 & Torch & [1, 32, 10, 64] \\
\hline 

contiguous & Memory Op & Llama-2 & Torch.Tensor & [1, 10, 32, 128], [1, 118, 32, 128] \\
\hline 

squeeze & Memory Op & Llama-2 & Torch &  [1, 1, 10, 128] \\ 
\hline 

GELU & Activation & GPT2-XL & transformers.activations & [1, 8, 6400] \\
\hline 

TrueDiv &Arithmetic& GPT2-XL & Torch & [1, 25, 8, 8] \\
\hline 

Split & Memory OP & GPT2-XL & Torch &[1, 8, 4800] \\ 
\hline 

view & Memory OP & GPT2-XL & Torch.Tensor & [1, 8, 1600]\\
\hline 

permute & Memory OP & GPT2-XL & Torch & [1, 8, 25, 64]\\
\hline 

reshape & Memory OP & ViT-b16 & Torch &  [1, 768, 14, 14]\\
\hline 

permute & Memory OP & ViT-b16 & Torch & [1, 768, 196] \\ 
\hline 

expand & Memory OP& ViT-b16 & Torch.Tensor & [1, 1, 768] \\
\hline 




\end {tabular}

\label{tab:microbench}
\caption{This table shows shows some of the NonGEMM operators collected while running \bench profiler. It categorizes each operator and provides input tensor size  examples.}
\end{table}
\end{center}

==> Tables/tab_model_table_fixed.tex <==
\begin{table}
    

% \caption{Tasks and Models in \bench}
\caption {Tasks and Models Evaluated in \autoref{sec:case_studies}}
\centering

\scriptsize
\begin{tabular} { |c|c|c|c |} 
\hline
%
% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Domain  \\  
% \end{tabular}} 
% & 

%
% \textbf{ Domain }  &
\textbf{ Application }  & \textbf{ Models }  & \textbf{ \# Params }  & \textbf{ Dataset } \\
\hline

% \multirow{13}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Computer  \\ Vision 
% \end{tabular}
% } &
\multirow{7}{*}{
\begin{tabular}[c]{@{}c@{}} 
Image \\ Classification (IC)
\end{tabular} 
}
& ViT base (Vt-b)~\cite{kolesnikov2021ViT}  & 307M 
& \multirow{7}{*}{
\begin{tabular}[c]{@{}c@{}} 
ImageNet \\ ~\cite{imagenet_cvpr09}
\end{tabular} 
}
\\ 
\cline{2-3}
% 
& ViT large (Vt-l)~\cite{kolesnikov2021ViT}  & 307M 
&
\\ 
\cline{2-3}
% 
& ViT huge (Vt-h)~\cite{kolesnikov2021ViT}  & 632M &  \\ 
\cline{2-3}
% 
& Swin tiny (Sw-t)~\cite{liu2021swin} & 29M &  \\ 
\cline{2-3}
% 
& Swin small (Sw-s)~\cite{liu2021swin} & 50M &  \\ 
\cline{2-3}
% 
& Swin base (Sw-b)~\cite{liu2021swin} & 88M &  \\ 
\hline
% 
 \multirow{3}{*}{
\begin{tabular}[c]{@{}c@{}} 
Object \\ Detection (OD)
\end{tabular} 
} & FasterRCNN (FRCNN)~\cite{ren2015faster} & 42M & \multirow{3}{*}
{
\begin{tabular}[c]{@{}c@{}} 
COCO \\~\cite{lin2014microsoft}
\end{tabular} 
} \\
\cline{2-3}
& MaskRCNN (MRCNN)~\cite{he2017mask} & 44M &  \\
\cline{2-3}
%
& DETR~\cite{carion2020end} & 41M & \\ 
\hline
%
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Image \\ Segmentation (IS)
\end{tabular}} & Maskformer (MF)~\cite{cheng2021per} & 102M & \multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
COCO \\~\cite{lin2014microsoft}
\end{tabular} 
}\\
%
\cline{2-3}
& SegFormer (Seg)~\cite{xie2021segformer} & 3.7M &  \\
\hline
% 
% \multirow{5}{*}{NLP} 
 \multirow{5}{*}{
\begin{tabular}[c]{@{}c@{}} 
Natural Language \\ Processing (NLP)
\end{tabular} 
} 
& GPT2~\cite{achiam2023gpt} & 117M & \multirow{5}{*}{
\begin{tabular}[c]{@{}c@{}} 
wikitext \\ ~\cite{wikitext}
\end{tabular} 
}
\\
\cline{2-3}
%
& GPT2 Large (gpt2-l)~\cite{achiam2023gpt} & 762M & \\
\cline{2-3}
%
& GPT2 X-Large (gpt2-xl)~\cite{achiam2023gpt} & 1.5B & \\
\cline{2-3}
%
& Llama 2-7B~\cite{touvron2023llama} & 7B & \\
\cline{2-3}
%
& Bert~\cite{kenton2019bert} & 110M & \\
\cline{2-3}
& Mixtral 8x7B~\cite{jiang2024mixtral} & 46.7B & \\
\hline
\end{tabular}
\label{tab:modeltable}
\vspace{-3mm}
\end{table}

==> Tables/tab_model_table_fixed_old.tex <==
\begin{table}
    

\caption{\bench Tasks and Models. \HK{Please add references for each model and the dataset}}

\centering

\scriptsize
\begin{tabular} { |c|c|c|c|c |} 
\hline
%
% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Domain  \\  
% \end{tabular}} 
% & 

%
\textbf{ Domain }  & \textbf{ Application }  & \textbf{ Models }  & \textbf{ \# Params }  & \textbf{ Dataset } \\
\hline

\multirow{13}{*}{
\begin{tabular}[c]{@{}c@{}} 
Computer  \\ Vision 
\end{tabular}
} & \multirow{8}{*}{
\begin{tabular}[c]{@{}c@{}} 
Image  \\ Classification 
\end{tabular}
} & ResNet50~\cite{he2016deep} & 0.85M & ImageNet~\cite{imagenet_cvpr09} \\
\cline{3-5}
%
& & MobileNetv2~\cite{sandler2018mobilenetv2} & 3.4M & ImageNet~\cite{imagenet_cvpr09} \\ 
\cline{3-5} 
%
&& ViT Base 16~\cite{kolesnikov2021ViT} & 86M & ImageNet~\cite{imagenet_cvpr09} \\ 
\cline{3-5} 
% 
&& ViT large 16~\cite{kolesnikov2021ViT}  & 307M & ImageNet~\cite{imagenet_cvpr09} \\ 
\cline{3-5} 
% 
&& ViT huge 14~\cite{kolesnikov2021ViT}  & 632M & ImageNet~\cite{imagenet_cvpr09} \\ 
\cline{3-5} 
% 
&& Swin tiny~\cite{liu2021swin} & 29M & ImageNet~\cite{imagenet_cvpr09} \\ 
\cline{3-5}
% 
&& Swin small~\cite{liu2021swin} & 50M & ImageNet~\cite{imagenet_cvpr09} \\ 
\cline{3-5}
% 
&& Swin base~\cite{liu2021swin} & 88M & ImageNet~\cite{imagenet_cvpr09} \\ 
\cline{2-5}
% 
& \multirow{3}{*}{
\begin{tabular}[c]{@{}c@{}} 
Object \\ Detection 
\end{tabular} 
} & FasterRCNN~\cite{ren2015faster} & 42M & COCO~\cite{lin2014microsoft} \\ 
\cline{3-5}
&& MaskRCNN~\cite{he2017mask} & 44M & COCO~\cite{lin2014microsoft} \\
\cline{3-5}
%
&& DETR~\cite{carion2020end} & 41M & COCO~\cite{lin2014microsoft} \\ 
\cline{2-5}
%
&\multirow{2}{*}{Segmentation} & Maskformer~\cite{cheng2021per} & 102M & COCO~\cite{lin2014microsoft}\\
\cline{3-5}
%
&& SegFormer~\cite{xie2021segformer} & 3.7M & COCO~\cite{lin2014microsoft} \\
\hline
% 
\multirow{5}{*}{NLP} & \multirow{5}{*}{
\begin{tabular}[c]{@{}c@{}} 
Language  \\ Models 
\end{tabular} 
} & GPT2~\cite{achiam2023gpt} & 117M & wikitext~\cite{wikitext} \\
\cline{3-5}
%
&& GPT2 Large~\cite{achiam2023gpt} & 762M & wikitext~\cite{wikitext} \\
\cline{3-5}
%
&& GPT2 X-Large~\cite{achiam2023gpt} & 1.5B & wikitext~\cite{wikitext} \\
\cline{3-5}
%
&& Llama 2-7B~\cite{touvron2023llama} & 7B & wikitext~\cite{wikitext} \\
\cline {3-5}
%
&& Bert~\cite{kenton2019bert} & 110M & wikitext~\cite{wikitext} \\
\hline
\end{tabular}
\label{tab:modeltable}

\end{table}

==> Tables/tab_models_ssm.tex <==
% % --- Table of Selected Models ---
% \begin{table}[h!]
% \centering
% \caption{The suite of models selected for characterization, categorized by architecture.
% %All models are evaluated in BF16 precision unless an INT4 version is specified.
% }
% \label{tab:model_zoo}
% \begin{tabular}{@{}llcc@{}}
% \toprule
% \textbf{Architecture} & \textbf{Model Name} & \textbf{Parameters} & \textbf{Quantized (precision)} \\ \midrule
% \multirow{4}{*}{Transformer} & Qwen2.5-0.5B & 0.5B & \checkmark(INT4/8) \\
% & Qwen2.5-1.5B & 1.5B & \checkmark(INT4/8) \\
% % & Qwen2.5-int4 & 494M & \checkmark \\
% & Phi-3-mini & 3.82B & \checkmark(INT4) \\
% & Llama-3.2 & 1B & \checkmark(INT4) \\
% & TinyLlama-v1 & 1.1B & \checkmark(INT4) \\
% & GPT-neo & 125m & N/A \\

% \midrule
% \multirow{3}{*}{SSM} & Mamba & 130M & \checkmark(INT4/8) \\
% & Mamba & 370M & \checkmark(INT4/8) \\
% & Mamba & 790M & \checkmark(INT4/8) \\
% & Mamba & 1.4B& \checkmark(INT4/8) \\
% & Mamba & 2.8B & \checkmark(INT4/8) \\
% & Mamba-2 & 130M & \checkmark(INT4/8) \\
% & Mamba-2 & 370M & \checkmark(INT4/8) \\
% & Mamba-2 & 780M & \checkmark(INT4/8) \\
% & Mamba-2 & 1.4B& \checkmark(INT4/8) \\
% & Mamba-2 & 2.8B & \checkmark(INT4/8) \\
% \midrule
% \multirow{2}{*}{Hybrid} & Zamba2 & 1.2B & N/A \\
% & Zamba2 & 2.7B & N/A \\
% & Hymba & 1.5B & N/A \\
% \bottomrule
% \end{tabular}
% \end{table}




\begin{table}[h!]
\centering
\caption{The suite of models selected for characterization.\\
\textbf{Quant.:} Availability of official INT4/8 checkpoints.}
\label{tab:model_zoo_short}
\resizebox{\columnwidth}{!}{% Resizes table to fit column width automatically
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Arch.} & \textbf{Family} & \textbf{Parameters (Sizes)} & \textbf{Quant.} \\ \midrule
\multirow{5}{*}{Trans.} & Qwen2.5 & 0.5B, 1.5B & \checkmark \\
 & Phi-3-mini & 3.82B & \checkmark \\
 & Llama-3.2 & 1B & \checkmark \\
 & TinyLlama & 1.1B & \checkmark \\
 & GPT-neo & 125M & -- \\ \midrule
\multirow{2}{*}{SSM} & Mamba & 130M, 370M, 790M, 1.4B, 2.8B & \checkmark \\
 & Mamba-2 & 130M, 370M, 780M, 1.4B, 2.8B & \checkmark \\ \midrule
\multirow{3}{*}{Hybrid} & Zamba2 & 1.2B, 2.7B & -- \\
 & Hymba & 1.5B & -- \\
 & Falcon-H1 & 0.5B, 1.5B & -- \\ \bottomrule
\end{tabular}%
}
\end{table}





==> Tables/tab_operator_group_summary.tex <==
\begin{center}
\begin{table}
\caption{Grouping non-GEMM operators based on Functionality}
\tiny
\begin{tabular} {| c | c | }
\hline 
\textbf{Operator Group} & \textbf{Description} \\
\hline 

Activation (Act) & Consists of linear and nonlinear activation functions  \\
\hline

Normalization (Norm)& Consists of different normalization functions \\
\hline

Softmax & Applies a function to map the features/logits to probabilities  \\ 
\hline 

Arithmetic (Arith) & Consists of operators performing element wise arithmetic operation on tensors\\
\hline

Memory Operations (MemOps) & Consists of operator performing allocating memory in different formats for tensors and returning different views and shapes of a tensor    \\ 
\hline 

NMS & Consists of non-maximum suppression functions used to filter out proposals \\ 

\hline 
%Embedding & Consists of the function performing the word and positional embedding in transformer based models\\  
%\hline 

\end {tabular}
\label{tab:operator_group_summary}
%\caption{Taxonomy for labeling and grouping NonGEMM operators.}

\end{table}
\end{center}
